A New Branching Bisimulation for Probabilistic Processes

We introduce a new branching bisimulation for probabilistic processes, which induces a more refined equivalence relation than any known equivalence that abstracts from unobservable actions, with a rooted version that is a congruence for a language of probabilistic process with the usual static as well as dynamic constructs including recursion.

==> Secs/3StrongBisimilarityCongruence.tex <==
\section{Strong Bisimilarity and Strong Congruence}\label{sec3}

Before defining what is a bisimulation, we need to lift a binary relation on $\mathcal{P}$ to a binary relation
on ${\sf Disc}({\mathcal P})$. Extensive research has already been conducted in this area, as seen in references ~\cite{LarsenS89,DengGHM09,Deng18,Jonsson0L01,CastiglioniT20}, among others. In this paper, we directly adopt the definition of relation lifting from reference~\cite{DengGHM09,Deng18}.

\begin{definition}\label{lifting-relation} Let $R\subseteq{\mathcal P}\times{\mathcal P}$ be a binary relation on
the set of processes. The lifting of $R$, written $R^\dagger$, is the smallest binary relation on
${\sf Disc}({\mathcal P})$ that satisfies:
\begin{enumerate}
\item $PR\,Q$ implies $\delta(P)R^\dagger\delta(Q)$;
\item $\Delta_iR^\dagger\Theta_i$ for $i\in I$ implies
$(\Sigma_{i\in I}p_i\Delta_i)R^\dagger(\Sigma_{i\in I}p_i\Theta_i)$,
where $I$ is an index set s.t.
$\Sigma_{i\in I}p_i=1$.
\end{enumerate}
\end{definition}

The following proposition is often used as an alternative definition of lifting. It is used in many proofs~\cite{BaierEM00,Hennessy12,DengH13}.

\begin{proposition}\label{Prop-DefofLifting}
Let $\Delta,\Theta\in{\sf Disc}(\mathcal{P})$, and $R\subseteq{\mathcal P}\times{\mathcal P}$.
Then the following are equivalent conditions:
\begin{enumerate}
\item $\Delta\,R^\dagger\,\Theta$.
%\item $\delta(P)\,R^\dagger\,\Theta$ iff $P R Q$ for all $Q \in \lceil\Theta\rceil$.
\item there exist $P_1,\ldots,P_n,Q_1,\ldots,Q_n\in\mathcal{P}$ and
$p_1,\ldots,p_n\in(0,1]$ such that $\Sigma_{i=1}^np_i=1$ and $P_i\,R\,Q_i$ for $i=1,\ldots,n$ and
$\Delta,\Theta$ can be decomposed as follows:
\begin{enumerate}
\item $\Delta=\Sigma_{i=1}^np_i\delta(P_i)$;
\item $\Theta=\Sigma_{i=1}^np_i\delta(Q_i)$.
%\item For aech $i\in\{1,2,\cdots,n\}$ we have $P_iRQ_i$.
\end{enumerate}
\item there exists a weight function $w:\mathcal{P}\times\mathcal{P}\rightarrow [0,1]$ such that
whenever $w(P,Q)>0$ then $PRQ$, and moreover
\begin{enumerate}
\item for all $P\in\mathcal{P}$ it holds that $\Sigma_{Q\in\mathcal{P}}w(P,Q)=\Delta(P)$;
\item for all $Q\in\mathcal{P}$ it holds that $\Sigma_{P\in\mathcal{P}}w(P,Q)=\Delta(Q)$.
%\item For aech $i\in\{1,2,\cdots,n\}$ we have $P_iRQ_i$.
\end{enumerate}
\end{enumerate}
\end{proposition}

The proof of this proposition and that of the following two proposition
about lifting can be found in \cite{deng15}.

\begin{proposition}\label{LeftDecomposable} (Left-Decomposable)
Let $R\subseteq\mathcal{P}\times\mathcal{P}$, $\Sigma_{i=1}^np_i=1$,
$\Delta_1,\ldots,\Delta_n\in{\sf Disc}(\mathcal{P})$.
If $(\Sigma_{i=1}^np_i\Delta_i)R^\dagger\Theta$, then $\Theta=\Sigma_{i=1}^np_i\Theta_i$
for some $\Theta_1,\ldots,\Theta_n\in{\sf Disc}(\mathcal{P})$ such that $\Delta_iR^\dagger\,\Theta_i$ for $i=1,\ldots,n$.
\end{proposition}

\begin{proposition}\label{Prolift}
	Let $R_1,R_2\subseteq\mathcal{P}\times\mathcal{P}.$
\begin{enumerate}
\item If $R_1\subseteq R_2$ then $R_1^\dagger\subseteq R_2^\dagger$.
\item $(R_1\cdot R_2)^\dagger=R_1^\dagger\cdot R_2^\dagger$.
%\item If $R$ is a transitive relation, then so is $R^\dagger$.
\end{enumerate}
\end{proposition}

The following  definition of strong bisimulation is a common
version of strong bisimulation for probabilistic processes, for example~\cite{deng15,Jonsson01}.
This version of bisimulation is different from a weaker version of {\em probabilistic bisimulation} in
that it matches a transition step by an individual transition instead of a {\em combined transition}
which is a combination of several transitions.

\begin{definition}\label{Strongbisim}
A symmetric  binary relation $R\subseteq\mathcal{P}\times\mathcal{P}$ is
a {\em strong bisimulation} if $P{R}\,Q$ implies that whenever
$P\arrow{\alpha}\Delta$
for some $\alpha\in{Act}$ and $\Delta\in{\sf Disc}(\mathcal{P})$, then there exists
$\Theta\in{\sf Disc}(\mathcal P)$ such that $Q\arrow{\alpha}\Theta$ and $\Delta\, R^\dagger\Theta$.

We say that two processes $P,Q\in\mathcal P$ are strong bisimilar, written $P\sim Q$,
if there is a strong bisimulation $R$ such that $PR\,Q$.
\end{definition}

The relation $\sim$ is called strong bisimilarity, and it is the union of all strong bisimulation relations. Next, we will prove that strong bisimilarity is itself an equivalence relation. Prior to this, we establish three useful properties of strong bisimulation relations through Proposition~\ref{Allstrongbisim}.

\begin{proposition}\label{Allstrongbisim}
Assume that each $R_i$ ($i\in I$) is a strong bisimulation, then the following relations
are all strong bisimulations:
\begin{enumerate}
\item ${\mathcal Id}_{\mathcal{P}}$ (defined as $\setof{(P,P)}{P\in\mathcal{P}}$),
\item $R_1\cdot R_2\cup R_2\cdot R_1$,
\item $\bigcup_{i\in I}R_i$.
\end{enumerate}
\end{proposition}
\begin{proof}
	The proof of 1): for $(P,P) \in {\mathcal Id}_{\mathcal{P}}$, whatever transition $P$ performs
say. $P\arrow{\alpha}\Delta$, the other $P$ in the pair can do exactly the same transition $P\arrow{\alpha}\Delta$ with $(\Delta,\Delta) \in ({\mathcal Id}_{\mathcal{P}})^\dagger$.

	The proof of 2): Suppose $(P,Q) \in R_1\cdot R_2\cup R_2\cdot R_1$ and $P\arrow{\alpha}\Delta$. We need to
show that there exists $\Theta$ such that $Q\arrow{\alpha}\Theta$ and
$\Delta(R_1\cdot R_2\cup R_2\cdot R_1)^\dagger\Theta$. We show this for $(P,Q)\in R_1\cdot R_2$, and
for $(P,Q)\in R_2\cdot R_1$ it can be done analogously. So Assume $(P,Q)\in R_1\cdot R_2$ and $P\arrow{\alpha}\Delta$,
then there exists $P'$ such that $(P,P') \in R_1$ and $(P',Q) \in R_2$; as $(P,P') \in R_1$ and
$R_1$ is a strong bisimulation,  $P\arrow{\alpha}\Delta$ implies that there exists
$\Delta'$ such that $P'\arrow{\alpha}\Delta'$ with $(\Delta,\Delta') \in R^\dagger_1$. And as $(P',Q) \in R_2$
and $R_2$ is a strong bisimulation, $P'\arrow{\alpha}\Delta'$ implies that there exists $\Theta$ such that
$Q\arrow{\alpha}\Theta$ with $(\Delta',\Theta) \in R^\dagger_2$. To sum up, for $(P,Q) \in R_1\cdot R_2$ and
$P\arrow{\alpha}\Delta$, we have found $\Theta$ such that $Q\arrow{\alpha}\Theta$ with
$(\Delta,\Theta)\in R^\dagger_1 \cdot R^\dagger_2$. By 2) of Proposition \ref{Prolift},
$(\Delta,\Theta)\in (R_1 \cdot R_2)^\dagger$, and by 1) of Proposition \ref{Prolift},
$(\Delta,\Theta)\in (R_1 \cdot R_2\cup R_2\cdot R_1)^\dagger$ as required.

The proof of 3): Assume $(P,Q) \in \bigcup_{i\in I}R_i$; then, there exists $j\in I$ s.t. $(P,P')$ belongs to some strong bisimulation $R_j$. If $P\arrow{\alpha}\Delta$, then there must exist $\Theta$ s.t. $Q\arrow{\alpha}\Theta$
with $(\Delta,\Theta) \in R^\dagger_j$. Hence $(\Delta,\Theta)\in (\bigcup_{i\in I}R_i)^\dagger$ as
$R_j^\dagger \subseteq (\bigcup_{i\in I}R_i)^\dagger$ by 1) of Proposition \ref{Prolift}.
% $R_j^\dagger \subseteq (\bigcup_{i\in I}R_i)^\dagger$, so $(\Delta,\Delta') \in (\bigcup_{i\in I}R_i)^\dagger$. So %$\bigcup_{i\in I}R_i$ is a strong bisimulation.
\end{proof}

\begin{theorem}\label{Th-StrongBisimilarity}
$\sim$ is the largest strong bisimulation on $\mathcal{P}$, and $\sim$ is an equivalence relation.
\end{theorem}
\begin{proof}
	By 3) of Proposition \ref{Allstrongbisim}, $\sim$ is a strong bisimulation and includes any other such. Therefore, $\sim$ is the largest strong bisimulation.

By 1) of Proposition \ref{Allstrongbisim}, for any $P\in\mathcal{P}$, $P\sim P$, so $\sim$ is reflexive.
If $P\sim P'$ then $(P,P')\in R $ for some strong bisimulation $R$, and $R$ is symmetric by Definition \ref{Strongbisim}, it
follows that $(P',P)\in R$ and thus $P' \sim P$, so $\sim$ is symmetric.
If  $P\sim P'$ and $P' \sim Q$ then  $(P,P')\in R_1$ and  $(P',Q)\in R_2$ for some strong bisimulations
$R_1,R_2$. So $(P,Q)\in R_1\cdot R_2\subseteq R_1\cdot R_2\cup R_2\cdot R_1$, and
by 2) of Proposition \ref{Allstrongbisim} $R_1\cdot R_2\cup R_2\cup R_1$ is a strong bisimulation, thus $P\sim Q$, and $\sim$
is transitive. Hence $\sim$ is an equivalence relation.
\end{proof}
 
To conclude the section we state two theorems which claims that $\sim$ is a congruence relation of the language,
i.e. $\sim$ is preserved by all constructions of the language.

\begin{theorem}\label{strongcongruence} For $P,Q\in\mathcal{P}$, if $P\sim Q$ then the following hold:
\begin{enumerate}
\item $\alpha.(\biguplus_{i=1}^n\langle p_i\rangle P_i)\sim
\alpha.(\biguplus_{i=1}^n\langle p_i\rangle Q_i)$, where $P_j$ is $P$, $Q_j$ is $Q$, and $P_i\equiv Q_i$ for $i\not=j$;
\item $\Sigma_{i=1}^nP_i\sim\Sigma_{i=1}^nQ_i$, where $P_j$ is $P$, $Q_j$ is $Q$, and $P_i\equiv Q_i$ for $i\not=j$;
%\item $P|O\sim Q|O, O|P\sim O|Q$,  where $O\in\mathcal{P}$;
\item $P|O\sim Q|O$, where $O\in\mathcal{P}$;
\item $P\backslash L\sim Q\backslash L$, where $L\subseteq\mathcal{L}$;
\item $P[f]\sim Q[f]$, where $f$ is a relabeling function.
\end{enumerate}
\end{theorem}
\begin{proof}
\textbf{The proof of 1:}
From Definition~\ref{lifting-relation} and $P\sim Q$, we have that $\delta(P_j)(\sim)^\dagger\delta(Q_j)$.
Moreover, since $P_i\equiv Q_i$ for $i\not=j$, it follows that $\delta(P_i)(\sim)^\dagger\delta(Q_i)$ .
By Definition~\ref{lifting-relation}, we have that $(\Sigma_{i=1}^n p_i\delta(P_i))(\sim)^\dagger(\Sigma_{i=1}^np_i\delta(Q_i))$ .
Given the transition: $\alpha.(\biguplus_{i=1}^n\langle p_i\rangle P_i)\arrow{\alpha}\Sigma_{i=1}^n p_i\delta(P_i)$, we can infer that there is a corresponding transition: $\alpha.(\biguplus_{i=1}^n\langle p_i\rangle Q_i)\arrow{\alpha} \Sigma_{i=1}^np_i\delta(Q_i)$ such that $(\Sigma_{i=1}^n p_i\delta(P_i))(\sim)^\dagger(\Sigma_{i=1}^np_i\delta(Q_i))$.
Therefore, we conclude that $\alpha.(\biguplus_{i=1}^n\langle p_i\rangle P_i)\sim \alpha.(\biguplus_{i=1}^n\langle p_i\rangle Q_i)$.\\

\textbf{The proof of 2:}
Suppose there is $\Sigma_{i=1}^nP_i\arrow{\alpha}\Delta$ for some $\alpha\in Act$ and $\Delta\in Disc(\mathcal{P})$.
By Definition~\ref{Opsemantics}, this implies that there exists some $P_i$ such that $P_i\arrow{\alpha}\Delta$.
If $i=j$, since $P\sim Q$, $P_j$ is $P$, $Q_j$ is $Q$, and $\sim$ is a strong bisimulation, there exists $Q_j\arrow{\alpha}\Theta$ such that $\Delta(\sim)^\dagger\Theta$.
Thus, by Definition~\ref{Opsemantics}, we have $\Sigma_{i=1}^nQ_i\arrow{\alpha}\Theta$ and $\Delta(\sim)^\dagger\Theta$ .
If $i\not=j$, given $P_i\equiv Q_i$, it follows that $Q_i\arrow{\alpha}\Delta$ and $\Delta(\sim)^\dagger\Delta$ trivially holds.
Thus, in bose cases, there exists $Q_i\arrow{\alpha}\Theta$ such that $\Delta(\sim)^\dagger\Theta$.
Therefore, by Definition~\ref{Opsemantics}, we have $\Sigma_{i=1}^nQ_i\arrow{\alpha}\Theta$ and $\Delta(\sim)^\dagger\Theta$ .
Hence, by Definition~\ref{Strongbisim}, we conclude that $\Sigma_{i=1}^nP_i\sim \Sigma_{i=1}^nQ_i$ . \\

\textbf{The proof of 3:}
To prove 3, it is sufficient to show that
$$R=\setof{(P|O,Q|O)}{P,Q,O\in\mathcal{P}, P\sim Q}$$
is a strong bisimulation. Since $\sim$ is an equivalence relation,  $R$ is clearly symmetric.
Suppose $(P|O,Q|O)\in R$ and $P|O\arrow{\alpha}\Delta$.
Then, according to Definition~\ref{Opsemantics}, we have three cases.\\

\textbf{Case 1:} In this case $P\arrow{\alpha}\Delta'$ %for $\Delta'=\Sigma_{P'\in\lceil\Delta'\rceil}\Delta'(P')\delta({P'})$
and
$\Delta= \Sigma_{P'\in\lceil\Delta'\rceil}\Delta'(P')\delta({P'|O})$.
Since $P\sim Q$, by Definition \ref{Strongbisim} there exists $\Theta'$ %=\Sigma_{Q'\in\lceil\Theta'\rceil}\Theta'(Q')\delta({Q'})$
such that
$Q\arrow{\alpha}\Theta'$ and $\Delta'(\sim)^\dagger \Theta'$.
Then, by Definition~\ref{Opsemantics} \textbf{Com}$_1$, there is $\Theta=\Sigma_{Q'\in\lceil\Theta'\rceil}\Theta'(Q')\delta({Q'|O})$ such that
$Q|O\arrow{\alpha}\Theta$.

From the 3 of Proposition~\ref{Prop-DefofLifting} and $\Delta'(\sim)^\dagger \Theta'$, there is a function
$w:\mathcal{P}\times \mathcal{P}\rightarrow [0,1]$ s.t.
\begin{enumerate}
\item[a)]$P'\sim Q'$ for all $w(P',Q')>0$,
\item[b)]$\Delta'(P')=\Sigma_{Q'\in\mathcal{P}}w(P',Q')$ for all $P'\in \mathcal{P}$, and
\item[c)]$\Theta'(Q')=\Sigma_{P'\in\mathcal{P}}w(P',Q')$ for all $Q'\in \mathcal{P}$.
\end{enumerate}
Let
$$\Delta^*=\Sigma_{P'\sim Q'}w(P',Q')\delta{(P'|O)},\Theta^*=\Sigma_{P'\sim Q'}w(P',Q')\delta{(Q'|O)}
$$
then since $(P'|O,Q'|O)\in R$ for $P'\sim Q'$, and
$$ \Sigma_{P'\sim Q'}w(P',Q')=\Sigma_{P'\in\mathcal{P}, Q'\in\mathcal{P}}w(P',Q')=\Sigma_{P'\in\mathcal{P}}\Sigma_{Q'\in\mathcal{P}}w(P',Q')=\Sigma_{P'\in\mathcal{P}}\Delta'(P')=1$$
(the first equality is because $w(P',Q')=0$ for $P'\not\sim Q'$, and the third is because b) above)
then by 1), 2) of Proposition~\ref{Prop-DefofLifting} $\Delta^*\;R^\dagger\;\Theta^*$, and
moreover we have
the following calculations:
$$\begin{array}{lclr}
\Delta&=&\Sigma_{P'\in\lceil\Delta'\rceil}\Delta'(P')\delta({P'|O})& \mbox{construction of $\Delta$}\\
&=&\Sigma_{P'\in\mathcal{P}}\Delta'(P')\delta({P'|O})& \mbox{$\Delta'(P')=0$
for $P'\notin\lceil\Delta'\rceil$}\\
&=&
\Sigma_{P'\in\mathcal{P}}(\Sigma_{Q'\in\mathcal{P}}w(P',Q'))\delta({P'|O})&\mbox{above b)}\\
&=&
\Sigma_{P'\in\mathcal{P},Q'\in\mathcal{P}}w(P',Q')\delta({P'|O})\\
&=&
\Sigma_{P'\sim Q'}w(P',Q')\delta({P'|O})&\mbox{by a) above, $w(P',Q')=0$ for $P'\not\sim Q'$}\\
&=&\Delta^*\\
\Theta&=&\Sigma_{Q'\in\lceil\Theta'\rceil}\Theta'(Q')\delta({Q'|O})& \mbox{construction of $\Theta$}\\
&=&\Sigma_{Q'\in\mathcal{P}}\Theta'(Q')\delta({Q'|O})& \mbox{$\Theta'(Q')=0$
for $Q'\notin\lceil\Theta'\rceil$}\\
&=&
\Sigma_{Q'\in\mathcal{P}}(\Sigma_{P'\in\mathcal{P}}w(P',Q'))\delta({Q'|O})&\mbox{above c)}\\
&=&
\Sigma_{P'\in\mathcal{P},Q'\in\mathcal{P}}w(P',Q')\delta({Q'|O})\\
&=&
\Sigma_{P'\sim Q'}w(P',Q')\delta({Q'|O})&\mbox{$w(P',Q')=0$ for $P'\not\sim Q'$}\\
&=&\Theta^*
\end{array}
$$
Thus, $\Delta R^\dagger \Theta$, as required. \\

\textbf{Case 2:} The transition of $P|O \arrow{\alpha} \Delta$ is due to
$O \arrow{\alpha} \Delta_1$ with 
$\Delta = \Sigma_{O'\in\lceil\Delta_1\rceil}\Delta_1(O')\delta({P|O'})$ by Definition~\ref{Opsemantics} \textbf{Com}$_2$.
Then by Definition~\ref{Opsemantics} \textbf{Com}$_2$, we also have $Q|O \arrow{\alpha} \Theta$ where
$\Theta = \Sigma_{O'\in\lceil\Delta_1\rceil}\Delta_1(O')\delta({Q|O'})$.
Given $P\sim Q$, it follows that $ P|O' R Q|O'$ from the definition of $R$.
Consequently, we obtain $ \delta(P|O') R^\dagger \delta(Q|O')$ by Definition~\ref{lifting-relation}.\\
Therefore, by Definition~\ref{lifting-relation}, we have $\Sigma_{O'\in\lceil\Delta_1\rceil}\Delta_1(O')\delta({P|O'}){R}^\dagger\Sigma_{O'\in \lceil\Delta_1\rceil}\Delta_1(O')\delta(Q|O')$, which simplifies to $\Delta R^\dagger\Theta$, as required.\\

\textbf{Case 3:} In this case, $\alpha=\tau$ and the
process undergoes a $\tau$ transition triggered by handshake synchronization, i.e.
there exists $\Delta',\Omega\in{\sf Disc}({\mathcal P})$ and $l\in\mathcal{A}\cup\overline{\mathcal{A}}$ such that $P\arrow{l}\Delta', O\arrow{\bar l}\Omega$, and
$\Delta=\Sigma_{(U,V)\in\lceil\Delta'\rceil\times\lceil\Omega\rceil}
(\Delta'(U)\cdot\Omega(V))\delta(U|V)$. Since $P \sim Q$, there exists $\Theta'$ such that $Q \arrow{l} \Theta'$ and
 $\Delta'(\sim)^\dagger \Theta'$.
Then, by Definition~\ref{Opsemantics}, $Q|O\arrow{\tau}\Theta$ where
$\Theta=\Sigma_{(W,V)\in\lceil\Theta'\rceil\times\lceil\Omega\rceil}
(\Theta'(W)\cdot\Omega(V))\delta(W|V)$. Now we only need to show that $\Delta R^\dagger\Theta$
to establish the case.

From the 3 of Proposition~\ref{Prop-DefofLifting} and $\Delta'(\sim)^\dagger \Theta'$, there is a function $w:\mathcal{P}\times\mathcal{P}\rightarrow [0,1]$ s.t.
\begin{enumerate}
\item[a)]$U\sim W$ for all $w(U,W)>0$,
\item[b)]$\Delta'(U)=\Sigma_{W\in\mathcal{P}}w(U,W)$ for all $U\in\mathcal{P}$, and
\item[c)]$\Theta'(W)=\Sigma_{U\in\mathcal{P}}w(U,W)$ for all $W\in \mathcal{P}$.
\end{enumerate}
For each $V\in\lceil\Omega\rceil$, let
%$$\Delta_V=\Sigma_{U\sim W}
%\Delta'(U)\delta(U|V), \ \Theta_V=\Sigma_{U\sim W}
%\Theta'(W)\delta(W|V),
%$$
$$\Delta_V=\Sigma_{U\sim W}w(U,W)\delta(U|V), \ \Theta_V=\Sigma_{U\sim W}w(U,W)\delta(W|V),
$$
then $(U|V,W|V)\in R$ for $U\sim W$, and
$$\Sigma_{U\sim W}w(U,W)=
\Sigma_{U\in\mathcal{P},W\in\mathcal{P}}w(U,W)=\Sigma_{U\in\mathcal{P}}\Sigma_{W\in\mathcal{P}}w(U,W)=
\Sigma_{U\in\mathcal{P}}\Delta'(U)=1,$$
then
by 1), 2) of Proposition~\ref{Prop-DefofLifting}
$\Delta_VR^\dagger\Theta_V$, so
$\Sigma_{V\in\lceil\Omega\rceil}\Omega(V)\Delta_VR^\dagger\Sigma_{V\in\lceil\Omega\rceil}\Omega(V)\Theta_V$, and
moreover we have
the following calculation:
$$\begin{array}{lclr}
\Delta&=&\Sigma_{(U,V)\in\lceil\Delta'\rceil\times\lceil\Omega\rceil}
(\Delta'(U)\cdot\Omega(V))\delta(U|V)& \mbox{construction of $\Delta$}\\
&=&\Sigma_{V\in\lceil\Omega\rceil}\Sigma_{U\in\lceil\Delta'\rceil}
(\Delta'(U)\cdot\Omega(V))\delta(U|V)\\
&=&\Sigma_{V\in\lceil\Omega\rceil}\Omega(V)\Sigma_{U\in\lceil\Delta'\rceil}
\Delta'(U)\delta(U|V)\\
&=&\Sigma_{V\in\lceil\Omega\rceil}\Omega(V)\Sigma_{U\in\mathcal{P}}
\Delta'(U)\delta(U|V)&\mbox{$\Delta'(U)=0$
for $U\notin\lceil\Delta'\rceil$}\\
&=&\Sigma_{V\in\lceil\Omega\rceil}\Omega(V)\Sigma_{U\in\mathcal{P}}
\Sigma_{W\in\mathcal{P}}w(U,W)\delta(U|V)&\mbox{above b)}\\
&=&\Sigma_{V\in\lceil\Omega\rceil}\Omega(V)\Sigma_{U\in\mathcal{P},
W\in\mathcal{P}}w(U,W)\delta(U|V)\\
&=&\Sigma_{V\in\lceil\Omega\rceil}\Omega(V)\Sigma_{U\sim W}w(U,W)\delta(U|V)&\mbox{$w(U,W)=0$ for $U\not\sim W$}\\
&=&\Sigma_{V\in\lceil\Omega\rceil}\Omega(V)\Delta_V\\

\Theta&=&\Sigma_{(W,V)\in\lceil\Theta'\rceil\times\lceil\Omega\rceil}
(\Theta'(W)\cdot\Omega(V))\delta(W|V)& \mbox{construction of $\Theta$}\\
&=&\Sigma_{V\in\lceil\Omega\rceil}\Sigma_{W\in\lceil\Theta'\rceil}
(\Theta'(W)\cdot\Omega(V))\delta(W|V)\\
&=&\Sigma_{V\in\lceil\Omega\rceil}\Omega(V)\Sigma_{W\in\lceil\Theta'\rceil}
\Theta'(W)\delta(W|V)\\
&=&\Sigma_{V\in\lceil\Omega\rceil}\Omega(V)\Sigma_{W\in\mathcal{P}}
\Theta'(W)\delta(W|V)&\mbox{$\Theta'(W)=0$
	for $W\notin\lceil\Theta'\rceil$}\\
&=&\Sigma_{V\in\lceil\Omega\rceil}\Omega(V)\Sigma_{W\in\mathcal{P}}
\Sigma_{U\in\mathcal{P}}w(U,W)\delta(W|V)&\mbox{above c)}\\
&=&\Sigma_{V\in\lceil\Omega\rceil}\Omega(V)\Sigma_{W\in\mathcal{P},
	U\in\mathcal{P}}w(U,W)\delta(W|V)\\
&=&\Sigma_{V\in\lceil\Omega\rceil}\Omega(V)\Sigma_{U\sim W}w(U,W)\delta(W|V)&\mbox{$w(U,W)=0$ for $U\not\sim W$}\\
&=&\Sigma_{V\in\lceil\Omega\rceil}\Omega(V)\Theta_V\\
\end{array}
$$
Thus $\Delta R^\dagger\Theta$.\\

\textbf{The proof of 4:} It suffices to show that
$$R=\setof{(P\backslash L,Q\backslash L)}{P\sim Q, P,Q\in\mathcal{P}}
$$
is a strong bisimulation. Since $\sim$ is an equivalence relation,  $R$ is clearly symmetric.

Assume $(P\backslash L,Q\backslash L)\in R$ and $P\backslash L\arrow{\alpha}\Delta$ .
Then, by Definition~\ref{Opsemantics}, there exists a transition
$P\arrow{\alpha}\Delta'$ with $\alpha \notin L\cup\overline{L}$ such that
$\Delta= \Sigma_{P'\in\lceil\Delta'\rceil}\Delta'(P')\delta({P'\backslash L})$ .
Since $P\sim Q$, by Definition \ref{Strongbisim} there exists $\Theta'=\Sigma_{Q'\in\lceil\Theta'\rceil}\Theta'(Q')\delta({Q'})$ such that
$Q\arrow{\alpha}\Theta'$ and $\Delta'(\sim)^\dagger \Theta'$.
Then, by Definition~\ref{Opsemantics}, there is $\Theta$ such that $Q \backslash L\arrow{\alpha}\Theta$ where $\Theta=\Sigma_{Q'\in\lceil\Theta'\rceil}\Theta'(Q')\delta({Q'\backslash L})$.
Now we only need to show that
$\Delta R^\dagger\Theta$ to establish the case. To this end,
from the 3 of Proposition~\ref{Prop-DefofLifting} and $\Delta'(\sim)^\dagger \Theta'$, there exists a function $w:\mathcal{P}\times\mathcal{P}\rightarrow [0,1]$ such that
\begin{enumerate}
	\item[a)] $P'\sim Q'$ for all $w(P',Q')>0$,
	\item[b)] $\Delta'(P')=\Sigma_{Q'\in\mathcal{P}}w(P',Q')$ for all $P'\in \mathcal{P}$, and
	\item[c)] $\Theta'(Q')=\Sigma_{P'\in\mathcal{P}}w(P',Q')$ for all $Q'\in \mathcal{P}$.
\end{enumerate}
Let $$\Delta^l=\Sigma_{P'\sim Q'}w(P',Q')\delta({P'\backslash L}),\
\Theta^l=\Sigma_{P'\sim Q'}w(P',Q')\delta({Q'\backslash L})$$
then
since $(P'\backslash L,Q'\backslash L)\in R$ for $P'\sim Q'$, and $$\Sigma_{P'\sim Q'}w(P',Q')=
\Sigma_{P'\in\mathcal{P},Q'\in\mathcal{P}}w(P',Q')=\Sigma_{P'\in\mathcal{P}}\Sigma_{Q'\in\mathcal{P}}w(P',Q')=
\Sigma_{P'\in\mathcal{P}}\Delta'(P')=1,$$
then
by 1), 2) of Proposition~\ref{Prop-DefofLifting}
$\Delta^lR^\dagger\Theta^l$, and
moreover we have
the following calculations:
$$\begin{array}{lclr}
	\Delta&=&\Sigma_{P'\in\lceil\Delta'\rceil}\Delta'(P')\delta({P'\backslash L})& \mbox{construction of $\Delta$}\\
	&=&\Sigma_{P'\in\mathcal{P}}\Delta'(P')\delta({P'\backslash L})& \mbox{$\Delta'(P')=0$
		for $P'\notin\lceil\Delta'\rceil$}\\
	&=&
	\Sigma_{P'\in\mathcal{P}}(\Sigma_{Q'\in\mathcal{P}}w(P',Q'))\delta({P'\backslash L})&\mbox{above b)}\\
	&=&
	\Sigma_{P'\in\mathcal{P},Q'\in\mathcal{P}}w(P',Q')\delta({P'\backslash L})\\
	&=&
	\Sigma_{P'\sim Q'}w(P',Q')\delta({P'\backslash L})&\mbox{$w(P',Q')=0$ for $P'\not\sim Q'$}\\
	&=&\Delta^l\\
	\Theta&=&\Sigma_{Q'\in\lceil\Theta'\rceil}\Theta'(Q')\delta({Q'\backslash L})& \mbox{construction of $\Theta$}\\
	&=&\Sigma_{Q'\in\mathcal{P}}\Theta'(Q')\delta({Q'\backslash L})& \mbox{$\Theta'(Q')=0$
		for $Q'\notin\lceil\Theta'\rceil$}\\
	&=&
	\Sigma_{Q'\in\mathcal{P}}(\Sigma_{P'\in\mathcal{P}}w(P',Q'))\delta({Q'\backslash L})&\mbox{above c)}\\
 	&=&
	\Sigma_{P'\in\mathcal{P},Q'\in\mathcal{P}}w(P',Q')\delta({Q'\backslash L})\\
	&=&
	\Sigma_{P'\sim Q'}w(P',Q')\delta({Q'\backslash L})&\mbox{$w(P',Q')=0$ for $P'\not\sim Q'$}\\
	&=&\Theta^l
\end{array}
$$
Thus $\Delta R^\dagger\Theta$.\\

\textbf{The proof of 5:} It is sufficient to show that
$$R=\setof{(P[f],Q[f])}{P,Q\in\mathcal{P},P\sim Q}
$$
is a strong bisimulation. Since $\sim$ is an equivalence relation, clearly $R$ is symmetric.

Suppose $(P[f],Q[f])\in R$ and $P[f]\arrow{\alpha}\Delta$.
Then, by Definition~\ref{Opsemantics}, there is a transition
$P\arrow{\beta}\Delta'$ such that
$\Delta= \Sigma_{P'\in\lceil\Delta'\rceil}\Delta'(P')\delta({P'[f]})$ and $\alpha=f[\beta]$.
Since $P\sim Q$, by Definition \ref{Strongbisim} there exists $\Theta'$
%=\Sigma_{Q'\in\lceil\Theta'\rceil}\Theta'(Q')\delta({Q'})$
such that
$Q\arrow{\beta}\Theta'$ and $\Delta'(\sim)^\dagger \Theta'$.
Then, by Definition~\ref{Opsemantics}, there is $\Theta$ such that $Q[f]\arrow{\alpha}\Theta$ where $\Theta=\Sigma_{Q'\in\lceil\Theta'\rceil}\Theta'(Q')\delta({Q'[f]})$. Now we only need to show that
$\Delta R^\dagger\Theta$ to establish the case. To this end,
from the 3 of Proposition~\ref{Prop-DefofLifting} and $\Delta'(\sim)^\dagger \Theta'$, there is a function
$w:\mathcal{P}\times\mathcal{P}\rightarrow [0,1]$ such that
\begin{enumerate}
\item[a)] $P'\sim Q'$ for all $w(P',Q')>0$,
\item[b)] $\Delta'(P')=\Sigma_{Q'\in\mathcal{P}}w(P',Q')$ for all $P'\in \mathcal{P}$, and
\item[c)] $\Theta'(Q')=\Sigma_{P'\in\mathcal{P}}w(P',Q')$ for all $Q'\in \mathcal{P}$.
\end{enumerate}
Let $$\Delta^f=\Sigma_{P'\sim Q'}w(P',Q')\delta({P'[f]}),\
\Theta^f=\Sigma_{P'\sim Q'}w(P',Q')\delta({Q'[f]})$$
then
since $(P'[f],Q'[f])\in R$ for $P'\sim Q'$, and $$\Sigma_{P'\sim Q'}w(P',Q')=
\Sigma_{P'\in\mathcal{P},Q'\in\mathcal{P}}w(P',Q')=\Sigma_{P'\in\mathcal{P}}\Sigma_{Q'\in\mathcal{P}}w(P',Q')=
\Sigma_{P'\in\mathcal{P}}\Delta'(P')=1,$$
then
by 1), 2) of Proposition~\ref{Prop-DefofLifting}
$\Delta^fR^\dagger\Theta^f$, and
moreover we have
the following calculations:
$$\begin{array}{lclr}
\Delta&=&\Sigma_{P'\in\lceil\Delta'\rceil}\Delta'(P')\delta({P'[f]})& \mbox{construction of $\Delta$}\\
&=&\Sigma_{P'\in\mathcal{P}}\Delta'(P')\delta({P'[f]})& \mbox{$\Delta'(P')=0$
for $P'\notin\lceil\Delta'\rceil$}\\
&=&
\Sigma_{P'\in\mathcal{P}}(\Sigma_{Q'\in\mathcal{P}}w(P',Q'))\delta({P'[f]})&\mbox{above b)}\\
&=&
\Sigma_{P'\in\mathcal{P},Q'\in\mathcal{P}}w(P',Q')\delta({P'[f]})\\
&=&
\Sigma_{P'\sim Q'}w(P',Q')\delta({P'[f]})&\mbox{$w(P',Q')=0$ for $P'\not\sim Q'$}\\
&=&\Delta^f\\
\Theta&=&\Sigma_{Q'\in\lceil\Theta'\rceil}\Theta'(Q')\delta({Q'[f]})& \mbox{construction of $\Theta$}\\
&=&\Sigma_{Q'\in\mathcal{P}}\Theta'(Q')\delta({Q'[f]})& \mbox{$\Theta'(Q')=0$
for $Q'\notin\lceil\Theta'\rceil$}\\
&=&
\Sigma_{Q'\in\mathcal{P}}(\Sigma_{P'\in\mathcal{P}}w(P',Q'))\delta({Q'[f]})&\mbox{above c)}\\
%&=&
%\Sigma_{Q'\in\lceil\Theta'\rceil,P'\in\lceil\Delta'\rceil}w(P',Q')\delta({Q'[f]})\\
%&=&
%\Sigma_{P'\in\lceil\Delta'\rceil,Q'\in\lceil\Theta'\rceil}w(P',Q'))\delta({Q'})\\
&=&
\Sigma_{P'\in\mathcal{P},Q'\in\mathcal{P}}w(P',Q')\delta({Q'[f]})\\
&=&
\Sigma_{P'\sim Q'}w(P',Q')\delta({Q'[f]})&\mbox{$w(P',Q')=0$ for $P'\not\sim Q'$}\\
&=&\Theta^f
\end{array}
$$
Thus $\Delta R^\dagger\Theta$.
\end{proof}

In process-calculus theory, bisimilarity is more than a definition of behavioural equivalence for systems: it also supplies a proof technique for establishing that two processes are equivalent. In principle, it suffices to exhibit a bisimulation relation that contains the pair of processes concerned.  However, every derived pair must also be checked, which makes proofs extremely heavy.  To ease this burden, Milner~\cite{milner89} introduced bisimulation up-to$\sim$, a relation that allows steps to be taken “up-to” known bisimilarity.  This idea was later generalised as the Up-to technique, subsequently studied extensively as an enhancement of the basic bisimulation proof method~\cite{Sangiorgi12,Sangiorgi24}.  In the sequel we extend the Up-to technology of CCS to the probabilistic setting and verify its soundness.

\begin{definition}
A symmetric  binary relation $R\subseteq\mathcal{P}\times\mathcal{P}$ is
a {\em strong bisimulation up to} $\sim$ if $P{R}\,Q$ implies that whenever
$P\arrow{\alpha}\Delta$
for some $\alpha\in{Act}$ and $\Delta\in{\sf Disc}(\mathcal{P})$, then there exists
$\Theta\in{\sf Disc}(\mathcal P)$ such that $Q\arrow{\alpha}\Theta$ and $\Delta\, (R\,\cdot\sim)^\dagger\Theta$.
\end{definition}

We now establish that the Up-to technique is sound for probabilistic processes: to show that two processes are strongly probabilistically bisimilar, it suffices to exhibit a strong bisimulation up-to$\sim$ that contains the pair.
More precisely, any relation $R$ which is a strong bisimulation up-to$\sim$ is already contained in strong bisimilarity.
This claim is formalised in Proposition~\ref{bisim-upto} below; its proof relies on Lemma\ref{bisim-upto lemma}.
Recall that $\sim\cdot\,R\,\cdot\sim$ denotes relational composition: $P(\sim\cdot\,R\,\cdot\sim)Q$ means there exist $P'$ and $Q'$ such that $P\sim P'$, $(P',Q')\in R$, and $Q'\sim Q$.

\begin{lemma} \label{bisim-upto lemma}
	If $R$ is a strong bisimulation up to $\sim$, then $\sim\cdot\,R\,\cdot\sim$ is a strong bisimulation.
\end{lemma}

\begin{proof}
Let $(P,Q)\in \sim\cdot\,R\,\cdot\sim$.
We have that there are $S_1,S_2\in \mathcal{P}$ such that $(P,S_1)\in \sim$, $(S_1,S_2)\in R$, and $(S_2,Q)\in \sim$.
Then, from Definition \ref{Strongbisim}, we get that whenever $P\arrow{\alpha}\Delta$ for some $\alpha\in{Act}$ and $\Delta\in{\sf Disc}(\mathcal{P})$, there is a $\Omega_1\in{\sf Disc}(\mathcal P)$ such that $$S_1\arrow{\alpha}\Omega_1\text{ and }\Delta\, (\sim)^\dagger\Omega_1.$$
At the same time, it can be implied that for $S_1\arrow{\alpha}\Omega_1$ there is a $\Omega_2\in{\sf Disc}(\mathcal P)$ such that
$$S_2\arrow{\alpha}\Omega_2\text{ and }\Omega_1\, (R\,\cdot\sim)^\dagger\Omega_2$$ from the definition of strong bisimulation up to and $(S_1,S_2)\in R$.
Moreover, for $S_2\arrow{\alpha}\Omega_2$, there is a $\Theta\in{\sf Disc}(\mathcal P)$ such that
$$Q\arrow{\alpha}\Theta\text{ and }\Omega_2\, (\sim)^\dagger\Theta$$
because of Definition \ref{Strongbisim} and $(S_2,Q)\in \sim$.
Thus, whenever $P\arrow{\alpha}\Delta$ there is a $\Theta\in{\sf Disc}(\mathcal P)$ such that $Q\arrow{\alpha}\Theta$ and $\Delta\, (\sim)^\dagger\cdot(R\,\cdot\sim)^\dagger\cdot(\sim)^\dagger\Theta$.
Then, from Proposition \ref{Prolift}, we have that $\Delta\, (\sim\,\cdot R\,\cdot\sim\,\cdot\sim)^\dagger\Theta$.
From Theorem \ref{Th-StrongBisimilarity}, $\sim\,\cdot\sim=\sim$ because $\sim$ is an equivalence relation.
Hence, whenever $P\arrow{\alpha}\Delta$ there is a $\Theta\in{\sf Disc}(\mathcal P)$ such that $Q\arrow{\alpha}\Theta$ and $\Delta\, (\sim\,\cdot R\,\cdot\sim)^\dagger\Theta$.
Therefore, $\sim\,\cdot R\,\cdot\sim$ is a strong bisimulation.
\end{proof}

\begin{proposition}\label{bisim-upto}
	 If $R$ is a strong bisimulation up to $\sim$, then $R\subseteq \sim$.
\end{proposition}
\begin{proof}
	By Lemma~{\ref{bisim-upto lemma}}, $\sim\cdot\,R\,\cdot\sim$ is a strong bisimulation, hence $\sim\cdot\,R\,\cdot\sim \subseteq \sim$ by Theorem~{\ref{Th-StrongBisimilarity}}.
	As the identity relation ${\mathcal Id}_{\mathcal{P}}\subseteq \sim$ by Proposition~{\ref{Allstrongbisim}},
	we have the relation $R={\mathcal Id}_{\mathcal{P}}\cdot\,R\,\cdot{\mathcal Id}_{\mathcal{P}}\subseteq \sim\cdot\,R\,\cdot\sim$, hence $R\subseteq \sim$ by transitivity.
\end{proof}

So far we have only defined the equivalence $\sim$ on processes, which are expressions without occurrence of variables.
To study whether $\sim$ is preserved under all construction of the language including recursive definition by equations,
we need $\sim$ to be general enough to compare expressions other than processes. Below, Definition~\ref{strongbisimilarbetweenopen} introduces strong bisimilarity between process expressions by reducing open expressions to closed processes: every variable occurring in an expression is simultaneously replaced by a closed process, thereby turning the expression into a fully specified, closed term.

\begin{definition}\label{strongbisimilarbetweenopen}
Let $E,F\in\mathcal{E}$ be two expressions, $\{X_1,\ldots,X_n\}$ contains all the variables occurring in $E$ and $F$.
We say that the expressions $E$ and $F$ are strongly bisimilar, notation $E\sim F$, if for all $P_1,\ldots,P_n\in\mathcal{P}$
we have that
$$E\{P_1/X_1,\ldots,P_n/X_n\}\sim F\{P_1/X_1,\ldots,P_n/X_n\}.
$$
\end{definition}

The next theorem states that $\sim$ is preserved by recursive definition.

\begin{theorem} \label{strongcongforrecur} Let $E_1,\ldots,E_n,F_1,\ldots,F_n$ be expressions containing variables
$\{X_1,\ldots,X_n\}$ at most. Let $A_1,\ldots,A_n,B_1,\ldots,B_n$ be constants with defining equations
\begin{equation}
	\nonumber
	\begin{split}
		A_i &\stackrel{{\rm def}}{=} E_i\{A_1/X_1, \ldots, A_n/X_n\} \\
		\text{and} \quad B_i &\stackrel{{\rm def}}{=} F_i\{B_1/X_1, \ldots, B_n/X_n\}
	\end{split}
\end{equation}
for $i=1,\ldots,n$.
If $E_i\sim F_i$ for $i=1,\ldots,n$, then $A_i\sim B_i$ for $i=1,\ldots,n$.
\end{theorem}
\begin{proof} We shall only prove the case in which there is a single recursive equation.
The same principle can be used to prove the general case. Thus assume
$$\begin{array}{ccl}
E&\sim &F\\
A&\stackrel{{\rm def}}{=} &E\{A/X\}\\
B&\stackrel{{\rm def}}{=} &F\{B/X\}
\end{array}
$$
and we shall prove that $A\sim B$. It will be enough to show that the relation $S\cup S^{-1}$
is a strong bisimulation
up to $\sim$, where $S$ is defined as follows:
$$S=\setof{(G\{A/X\},G\{B/X\})}{G\mbox{ contains at most variable }X}.
$$
For then, when $G\equiv X$, it follows that $A\sim B$ by proposition~{\ref{bisim-upto}}. Now to prove 
$S\cup S^{-1}$
is a strong bisimulation
up to $\sim$, by
symmetry, it is enough to prove the following statement:
\begin{center} if $G\{A/X\}\arrow{\alpha}\Delta$, then $G\{B/X\}\arrow{\alpha}\Theta$ with $\Delta\, (S\,\cdot\sim)^\dagger\Theta$.
\end{center}
For the sake of the subsequent argumentation, we first establish the following property of $S$.
\begin{claim}\label{S-property} $S$ is a congruence for process constructions, i.e.
\begin{enumerate}
\item If $(P_1,P_2)\in S$ and $(Q_1,Q_2)\in S$, then $(P_1|Q_1,P_2|Q_2)\in S$.
\end{enumerate}
\end{claim}

The proof of this property is routine, for example here we show that 
if $(P_1,P_2)\in S$ and $(Q_1,Q_2)\in S$, then $(P_1|Q_1,P_2|Q_2)\in S$.
Given $(P_1,P_2)\in S$ , there exists some $H_1$ such that $P_1=H_1\{A/X\}$ and $P_2=H_1\{B/X\}$. Likewise, since $(Q_1,Q_2)\in S$ , there exists some $H_2$ such that $Q_1=H_2\{A/X\}$ and $Q_2=H_2\{B/X\}$. Therefore, if we set $H \equiv H_1|H_2$, we have $(P_1|Q_1,P_2|Q_2) \equiv (H\{A/X\},H\{B/X\})\in S$.

With this property of $S$, we now turn to the proof of the main statement.
The proof proceeds by induction on the inference of $G\{A/X\}\arrow{\alpha}\Delta$. We examine the possible shapes of G.\\

\textbf{1) $G\equiv X$.} In this case, we have $G\{A/X\}\equiv A$ and $G\{B/X\}\equiv B$. We need to prove that for any transition from A, e.g., $A\arrow{\alpha}\Delta$, there exists a $\Theta$ such that $B\arrow{\alpha}\Theta$ with $\Delta\, ( S\,\cdot\sim)^\dagger\Theta$.
By hypothesis, $A\stackrel{{\rm def}}{=} E\{A/X\}$, suppose $A\arrow{\alpha}\Delta$,
also $E\{A/X\}\arrow{\alpha}\Delta$ ;
hence, induction can be applied to conclude that $E\{B/X\}\arrow{\alpha}\Theta'$ with $\Delta\, ( S\,\cdot\sim)^\dagger\Theta'$.
By $E \sim F$, there exists a $\Theta$ such that $F\{B/X\}\arrow{\alpha}\Theta$ with $\Theta' \sim^\dagger \Theta$.
Since $B\stackrel{{\rm def}}{=} F\{B/X\}$, we get  $B \arrow{\alpha}\Theta$.
By proposition~{\ref{Prolift}},$\Delta\, ( S\,\cdot\sim)^\dagger\Theta$ , as required.\\

\textbf{2) $G\equiv \alpha.\biguplus_{j\in J}\langle p_{j}\rangle G'_{j}$.}
In this case, $G\{A/X\}\equiv\alpha.\biguplus_{j\in J}\langle p_{j}\rangle G'_{j}\{A/X\} \arrow{\alpha} \Sigma_{j\in J}p_{j}\delta(G'_{j}\{A/X\})$.
Similarly, $G\{B/X\}\equiv\alpha.\biguplus_{j\in J}\langle p_{j}\rangle G'_{j}\{B/X\} \arrow{\alpha} \Sigma_{j\in J}p_{j}\delta(G'_{j}\{B/X\})$.
Since $(G'_{j}\{A/X\},G'_{j}\{B/X\})\in S$ for every $j\in J$, we get that $\Sigma_{j\in J}p_{j}\delta(G'_{j}\{A/X\}) S^ \dagger \Sigma_{j\in J}p_{j}\delta(G'_{j}\{B/X\})$ by Definition~{\ref{lifting-relation}}, as required.\\

\textbf{3) $G\equiv \sum_{i\in I}G'_{i}$.}
In this case, $G\{A/X\}\equiv\sum_{i\in I}G'_i\{A/X\}$, a transition from $G\{A/X\} $ is derivable on if $G'_n\{A/X\}\arrow{\alpha}\Delta$ for some $n\in I$.
Without loss of generality, assume the transition is due to $G'_1\{A/X\}$. By hypothesis, there exists a $\Theta$ such that $G'_1\{B/X\}\arrow{\alpha}\Theta$ with $\Delta\, (  S\,\cdot\sim)^\dagger\Theta$.
 By the operational semantics, this ensures that also $G\{B/X\}\equiv \sum_{i\in I}G'_i\{B/X\}\arrow{\alpha}\Theta$ with $\Delta\, ( S\,\cdot\sim)^\dagger\Theta$, as required.\\

\textbf{4) $G\equiv G_1|G_2$.} In this case, $G\{A/X\}\equiv G_1\{A/X\}|G_2\{A/X\}$. 
There are three cases for the action $G\{A/X\}\arrow{\alpha}\Delta$, according to whether it arises from one or other component alone or from a communication.
\\
\textbf{Case 1:} In this case, the $\alpha$ transition is due to $G_1\{A/X\}\arrow{\alpha}\Delta_1$ . Hence, by Definition~\ref{Opsemantics}, we have $\Delta=\Sigma_{P'\in\lceil\Delta_1\rceil}\Delta_1(P')\delta(P'|G_2\{A/X\})$ .
By the induction hypothesis, we have $G_1\{B/X\} \arrow{\alpha} \Delta_2$
with $\Delta_1 (S\,\cdot\sim)^\dagger \Delta_2$ . Then by definition~\ref{Opsemantics}, there exists $\Theta$ such that $G\{B/X\} \arrow{\alpha} \Theta$ where
$\Theta= \Sigma_{Q'\in\lceil\Delta_2\rceil}\Delta_2(Q')\delta(Q'|G_2\{B/X\})$.
Now we only need to show that
$\Delta(S\,\cdot\sim)^\dagger \Theta$ holds to establish the case. 
Since $\Delta_1 (S\,\cdot\sim)^\dagger \Delta_2$, there exists some $\Delta_3$ such that $\Delta_1 S^\dagger \Delta_3$ and $\Delta_3 (\sim)^\dagger \Delta_2$. Let
$\Theta'=\Sigma_{P''\in\mathcal{P}}\Delta_3(P'')\delta(P''|G_2\{B/X\})$. Then, to establish
$\Delta(S\,\cdot\sim)^\dagger \Theta$, it is sufficient to show that $\Delta S^\dagger\Theta'$ and $\Theta'(\sim)^\dagger \Theta$.
From 3 of Proposition~\ref{Prop-DefofLifting} and $\Delta_1 S^\dagger \Delta_3$,
there exists a function $w_1:\mathcal{P}\times\mathcal{P}\rightarrow [0,1]$ such that
\begin{enumerate}
	\item[a)] $P'S P''$ for all $w_1(P',P'')>0$,
	\item[b)] $\Delta_1(P')=\Sigma_{P''\in\mathcal{P}}w_1(P',P'')$ for all $P'\in \mathcal{P}$, and
	\item[c)] $\Delta_3(P'')=\Sigma_{P'\in\mathcal{P}}w_1(P',P'')$ for all $P''\in \mathcal{P}$.
\end{enumerate}
Then we have the following calculations:
$$\begin{array}{lclr}
	\Delta&=&\Sigma_{P'\in\lceil\Delta_1\rceil}\Delta_1(P')\delta(P'|G_2{A/X})&  \\
	&=&\Sigma_{P'\in\mathcal{P}}\Delta_1(P')\delta(P'|G_2\{A/X\})& \mbox{$\Delta_1(P')=0$
		for $P'\notin\lceil\Delta_1\rceil$}\\
	&=&
	\Sigma_{P'\in\mathcal{P}}(\Sigma_{P''\in\mathcal{P}}w_1(P',P''))\delta(P'|G_2\{A/X\})&\mbox{above b)}\\
	&=&
	\Sigma_{P'\in\mathcal{P},P''\in\mathcal{P}}w_1(P',P'')\delta(P'|G_2\{A/X\})\\
	&=&
	\Sigma_{P' S P''}w_1(P',P'')\delta(P'|G_2\{A/X\})&\mbox{$w_1(P',P'')=0$ for $(P',P'')\notin S $}\\
\end{array}
$$
Similarly, we can obtain
$\Theta'=\Sigma_{P' S P''}w_1(P',P'')\delta(P''|G_2\{B/X\})$.\\
Since $P'S P''$ and $G_2\{A/X\} S G_2\{B/X\}$, we have $(P'|G_2\{A/X\},P''|G_2\{B/X\})\in S$ by Claim~\ref{S-property}, thus $\Delta S^\dagger\Theta'$.

On the other hand, from 3 of Proposition~\ref{Prop-DefofLifting} and $\Delta_2 (\sim)^\dagger \Delta_3$,
there exists a function $w_2:\mathcal{P}\times\mathcal{P}\rightarrow [0,1]$ such that
\begin{enumerate}
	\item[a)] $Q'\sim P''$ for all $w_2(Q',P'')>0$,
	\item[b)] $\Delta_2(Q')=\Sigma_{P''\in\mathcal{P}}w_2(Q',P'')$ for all $Q'\in \mathcal{P}$, and
	\item[c)] $\Delta_3(P'')=\Sigma_{Q'\in\mathcal{P}}w_2(Q',P'')$ for all $P''\in \mathcal{P}$.
\end{enumerate}
Then we have the following calculations:
$$\begin{array}{lclr}
	\Theta&=&\Sigma_{Q'\in\lceil\Delta_2\rceil}\Delta_2(Q')\delta(Q'|G_2\{B/X\})&  \\
	&=&\Sigma_{Q'\in\mathcal{P}}\Delta_2(Q')\delta({Q'|G_2\{B/X\}})& \mbox{$\Delta_2(Q')=0$
		for $Q'\notin\lceil\Delta_2\rceil$}\\
	&=&
	\Sigma_{Q'\in\mathcal{P}}(\Sigma_{P''\in\mathcal{P}}w_2(Q',P''))\delta({Q'|G_2\{B/X\}})&\mbox{above b)}\\
	&=&
	\Sigma_{Q'\in\mathcal{P},P''\in\mathcal{P}}w_2(Q',P'')\delta({Q'|G_2\{B/X\}})\\
	&=&
	\Sigma_{Q' \sim P''}w_2(Q',P'')\delta(Q'|G_2\{B/X\})&\mbox{$w_2(Q',P'')=0$ for $(Q',P'')\not\sim S $}\\
\end{array}
$$
Similarly, we can obtain $\Theta'=\Sigma_{Q'\sim P''}w_2(Q',P'')\delta({P''|G_2{B/X}})$.
Since $Q'\sim P''$ , by congruence we have $(Q'|G_2\{B/X\})\sim(P''|G_2\{B/X\})$,  thus $\Theta(\sim)^\dagger\Theta'$, as required.
\\

\textbf{Case 2:} In contrast to Case 1, the $\alpha$ transition is due to $G_2\{A/X\}$.The proof of this case is similar to that of Case 1 and is thus omitted for brevity.\\

\textbf{Case 3:} We consider the case where $\alpha = \tau$, and we have $G_1\{A/X\}\arrow{l}\Delta_1$, and $G_2\{A/X\}\arrow{\bar{l}}\Delta_2$.
According to Definition~\ref{Opsemantics}, we have  $\Delta=\Sigma_{(U,V)\in\lceil\Delta_1\rceil\times\lceil\Delta_2\rceil}(\Delta_1(U)\cdot\Delta_2(V))\delta(U|V)$ .
Furthermore, based on the induction hypothesis, we have $G_1\{B/X\} \arrow{l} \Theta_1$
with $\Delta_1 (S\,\cdot\sim)^\dagger \Theta_1$, and $G_2\{B/X\} \arrow{\bar{l}} \Theta_2$
with $\Delta_2 (S\,\cdot\sim)^\dagger \Theta_2$.
Then by Definition~\ref{Opsemantics} again, there exists $\Theta$ such that $G\{B/X\} \arrow{\tau} \Theta$ where
$\Theta= \Sigma_{(U',V')\in\lceil\Theta_1\rceil\times\lceil\Theta_2\rceil}(\Theta_1(U')\cdot\Theta_2(V'))\delta(U'|V')$. Now we only need to show
$\Delta(S\,\cdot\sim)^\dagger \Theta$ to establish the case.\\
Since $\Delta_1 (S\,\cdot\sim)^\dagger \Theta_1$, there exists some $\Delta_1^{'}$ such that $\Delta_1 S^\dagger \Delta_1^{'} (\sim)^\dagger \Theta_1$ . In the same manner, since $\Delta_2 (S\,\cdot\sim)^\dagger \Theta_2$, there exists some $\Delta_2^{'}$ such that $\Delta_2 S^\dagger \Delta_2^{'} (\sim)^\dagger \Theta_2$ .
Let $\Delta'=\Sigma_{(U'',V'')\in\lceil\Delta_1^{'}\rceil\times\lceil\Delta_2^{'}\rceil}(\Delta_1^{'}(U'')\cdot\Delta_2^{'}(V''))\delta(U''|V'')$, then to establish $\Delta (\sim)^\dagger \Theta $
it is sufficient to show that $\Delta S^\dagger \Delta'$
and $\Delta' (\sim)^\dagger \Theta$.
From 3 of Proposition~\ref{Prop-DefofLifting} and $\Delta_1 S^\dagger \Delta_1^{'}$,
there exists a function $w_1:\mathcal{P}\times\mathcal{P}\rightarrow [0,1]$ such that
\begin{enumerate}
	\item[a)] $U S U''$ for all $w_1(U,U'')>0$,
	\item[b)] $\Delta_1(U)=\Sigma_{U''\in\mathcal{P}}w_1(U,U'')$ for all $U\in \mathcal{P}$, and
	\item[c)] $\Delta_1^{'}(U'')=\Sigma_{U\in\mathcal{P}}w_1(U,U'')$ for all $U''\in \mathcal{P}$.
\end{enumerate}
Following the same reasoning, from 3 of Proposition~\ref{Prop-DefofLifting} and $\Delta_2 S^\dagger \Delta_2^{'}$,
there exists a function $w_2:\mathcal{P}\times\mathcal{P}\rightarrow [0,1]$ such that
\begin{enumerate}
	\item[d)] $V S V''$ for all $w_2(V,V'')>0$,
	\item[e)] $\Delta_2(V)=\Sigma_{V''\in\mathcal{P}}w_2(V,V'')$ for all $V\in \mathcal{P}$, and
	\item[f)] $\Delta_2^{'}(V'')=\Sigma_{V\in\mathcal{P}}w_2(V,V'')$ for all $V''\in \mathcal{P}$.
\end{enumerate}	
Based on these definitions and conditions, we can proceed with the following calculations:
$$\begin{array}{lclr}
	\Delta&=&\Sigma_{(U,V)\in\lceil\Delta_1\rceil\times\lceil\Delta_2\rceil}(\Delta_1(U)\cdot\Delta_2(V))\delta(U|V)&  \\
	&=&\Sigma_{U\in\lceil\Delta_1\rceil}\Delta_1(U)\Sigma_{V\in\lceil\Delta_2\rceil}\Delta_2(V)\delta(U|V)&  \\
	&=&\Sigma_{U\in\mathcal{P}}\Delta_1(U)\Sigma_{V\in\lceil\Delta_2\rceil}\Delta_2(V)\delta(U|V)& \mbox{$\Delta_1(U)=0$ for $U\notin\lceil\Delta_1\rceil$}\\
	&=&\Sigma_{U\in\mathcal{P}}\Delta_1(U)\Sigma_{V\in\mathcal{P}}\Delta_2(V)\delta(U|V)& \mbox{$\Delta_2(V)=0$	for $V\notin\lceil\Delta_2\rceil$}\\
	&=&\mbox{\small$\Sigma_{U\in\mathcal{P}}(\Sigma_{U''\in\mathcal{P}}w_1(U,U''))\Sigma_{V\in\mathcal{P}}(\Sigma_{V''\in\mathcal{P}}w_2(V,V''))\delta(U|V)$}&\mbox{above b),e)}\\
	&=&\Sigma_{U\in\mathcal{P},U''\in\mathcal{P}}w_1(U,U'')\Sigma_{V\in\mathcal{P},V''\in\mathcal{P}}w_2(V,V'')\delta(U|V)\\
	&=&\Sigma_{U S U''}w_1(U,U'')\Sigma_{V\in\mathcal{P},V''\in\mathcal{P}}w_2(V,V'')\delta(U|V)&\mbox{$w_1(U,U'')=0$ for $(U,U'')\notin S $}\\
	&=&\Sigma_{U S U''}w_1(U,U'')\Sigma_{V S V''}w_2(V,V'')\delta(U|V)&\mbox{$w_2(V,V'')=0$ for $(V,V'')\notin S $}\\
\end{array}
$$
Similarly, we can obtain $\Delta'=\Sigma_{U S U''}w_1(U,U'')\Sigma_{V S V''}w_2(V,V'')\delta(U''|V'')$. By Claim~\ref{S-property}, we know that $(U|V,U''|V'')\in S$. Therefore, it follows that $\Delta S^\dagger \Delta'$.\\
Since $\Theta_1 (\sim)^\dagger \Delta_1^{'}$, from 3 of Proposition~\ref{Prop-DefofLifting},
there exists a function $w_3:\mathcal{P}\times\mathcal{P}\rightarrow [0,1]$ such that
\begin{enumerate}
	\item[g)] $U' \sim U''$ for all $w_3(U',U'')>0$,
	\item[h)] $\Delta_1^{'}(U'')=\Sigma_{U'\in\mathcal{P}}w_3(U',U'')$ for all $U''\in \mathcal{P}$, and
	\item[i)] $\Theta_1(U')=\Sigma_{U''\in\mathcal{P}}w_3(U',U'')$ for all $U'\in \mathcal{P}$.
\end{enumerate}
Similarly, since $\Theta_2 (\sim)^\dagger \Delta_2^{'}$, from 3 of Proposition~\ref{Prop-DefofLifting},there exists a function $w_4:\mathcal{P}\times\mathcal{P}\rightarrow [0,1]$ such that
\begin{enumerate}
	\item[j)] $V' \sim V''$ for all $w_4(V',V'')>0$,
	\item[k)] $\Delta_2^{'}(V'')=\Sigma_{V'\in\mathcal{P}}w_4(V',V'')$ for all $V''\in \mathcal{P}$, and
	\item[l)] $\Theta_2(V')=\Sigma_{V''\in\mathcal{P}}w_4(V',V'')$ for all $V'\in \mathcal{P}$.
\end{enumerate}
Next, We proceed with the following calculations:
$$\begin{array}{lclr}		
	\Theta&=&\Sigma_{(U',V')\in\lceil\Theta_1\rceil\times\lceil\Theta_2\rceil}(\Theta_1(U')\cdot\Theta_2(V'))\delta(U|V)&  \\
	&=&\Sigma_{U'\in\lceil\Theta_1\rceil}\Theta_1(U')\Sigma_{V'\in\lceil\Theta_2\rceil}\Theta_2(V')\delta(U'|V')&  \\
	&=&\Sigma_{U'\in\mathcal{P}}\Theta_1(U')\Sigma_{V'\in\lceil\Theta_2\rceil}\Theta_2(V')\delta(U'|V')& \mbox{$\Theta_1(U')=0$ for $U'\notin\lceil\Theta_1\rceil$}  \\
	&=&\Sigma_{U'\in\mathcal{P}}\Theta_1(U')\Sigma_{V'\in\mathcal{P}}\Theta_2(V')\delta(U'|V')& \mbox{$\Theta_2(V')=0$ for $V'\notin\lceil\Theta_2\rceil$}  \\
	&=&\mbox{\small$\Sigma_{U'\in\mathcal{P}}(\Sigma_{U''\in\mathcal{P}}w_3(U',U''))\Sigma_{V'\in\mathcal{P}}(\Sigma_{V''\in\mathcal{P}}w_4(V,V''))\delta(U'|V')$}&\mbox{above i),l)}\\
	&=&\Sigma_{U'\in\mathcal{P},U''\in\mathcal{P}}w_3(U',U'')\Sigma_{V'\in\mathcal{P},V''\in\mathcal{P}}w_4(V',V'')\delta(U'|V')\\
	&=&\Sigma_{U' \sim U''}w_3(U',U'')\Sigma_{V'\in\mathcal{P},V''\in\mathcal{P}}w_4(V',V'')\delta(U'|V')&\mbox{$w_3(U',U'')=0$ for $ U'\sim U''  $}\\
	&=&\Sigma_{U' \sim U''}w_3(U',U'')\Sigma_{V' \sim V''}w_4(V',V'')\delta(U'|V')&\mbox{$w_4(V',V'')=0$ for $V' \sim V'' $}\\
\end{array}
$$
Similarly, we can obtain $\Delta'=\Sigma_{U' \sim U''}w_3(U',U'')\Sigma_{V' \sim V''}w_4(V',V'') \delta(U''|V'')$.
Given that $U' \sim U''$ and $V' \sim V''$, it follows by congruence that $(U'|V')\sim(U''|V'')$. Consequently, we establish that $\Theta (\sim)^\dagger \Delta'$. This completes the proof.
\\
\textbf{5) $G\equiv G_1\backslash L$.} In this case, $G\{A/X\} \equiv G_1\{A/X\}\backslash L$.
Assume $G\{A/X\} \arrow{\alpha} \Delta$, then there exists a transition $G_1\{A/X\} \arrow{\alpha} \Delta_1$
with $\alpha \notin L\cup\overline{L}$ such that
$\Delta= \Sigma_{P'\in\lceil\Delta_1\rceil}\Delta_1(P')\delta({P'\backslash L})$.
By the induction hypothesis, we have $G_1\{B/X\} \arrow{\alpha} \Delta_2$
with $\Delta_1 (S\,\cdot\sim)^\dagger \Delta_2$ . Then by Definition~\ref{Opsemantics}, there exists $\Theta$ such that $G\{B/X\} \arrow{\alpha} \Theta$ where
$\Theta= \Sigma_{Q'\in\lceil\Delta_2\rceil}\Delta_2(Q')\delta({Q'\backslash L})$. Now we only need to show
$\Delta(S\,\cdot\sim)^\dagger \Theta$ to establish the case.
Since $\Delta_1 (S\,\cdot\sim)^\dagger \Delta_2$, there exists some $\Delta_3$ such that $\Delta_1 S^\dagger \Delta_3 (\sim)^\dagger \Delta_2$, and let
$\Theta'=\Sigma_{P''\in\mathcal{P}}\Delta_3(P'')\delta(P''\backslash L)$, then to establish
$\Delta(S\,\cdot\sim)^\dagger \Theta$ it is sufficient to show that $\Delta S^\dagger\Theta'(\sim)^\dagger \Theta$.
From 3 of Proposition~\ref{Prop-DefofLifting} and $\Delta_1 S^\dagger \Delta_3$,
there exists a function $w_1:\mathcal{P}\times\mathcal{P}\rightarrow [0,1]$ such that
\begin{enumerate}
	\item[a)] $P'S P''$ for all $w_1(P',P'')>0$,
	\item[b)] $\Delta_1(P')=\Sigma_{P''\in\mathcal{P}}w_1(P',P'')$ for all $P'\in \mathcal{P}$, and
	\item[c)] $\Delta_3(P'')=\Sigma_{P'\in\mathcal{P}}w_1(P',P'')$ for all $P''\in \mathcal{P}$.
\end{enumerate}
Then we have the following calculations:
$$\begin{array}{lclr}
	\Delta&=&\Sigma_{P'\in\lceil\Delta_1\rceil}\Delta_1(P')\delta(P'\backslash L)&  \\
	&=&\Sigma_{P'\in\mathcal{P}}\Delta_1(P')\delta({P'\backslash L})& \mbox{$\Delta_1(P')=0$
		for $P'\notin\lceil\Delta_1\rceil$}\\
	&=&
	\Sigma_{P'\in\mathcal{P}}(\Sigma_{P''\in\mathcal{P}}w_1(P',P''))\delta({P'\backslash L})&\mbox{above b)}\\
	&=&
	\Sigma_{P'\in\mathcal{P},P''\in\mathcal{P}}w_1(P',P'')\delta({P'\backslash L})\\
	&=&
	\Sigma_{P' S P''}w_1(P',P'')\delta({P'\backslash L})&\mbox{$w_1(P',P'')=0$ for $(P',P'')\notin S $}\\
\end{array}
$$
Similarly, we can obtain
$\Theta'=\Sigma_{P' S P''}w_1(P',P'')\delta({P''\backslash L})$, thus $\Delta S^\dagger\Theta'$.

On the other hand, from 3 of Proposition~\ref{Prop-DefofLifting} and $\Delta_2 (\sim)^\dagger \Delta_3$,
there exists a function $w_2:\mathcal{P}\times\mathcal{P}\rightarrow [0,1]$ such that
\begin{enumerate}
	\item[a)] $Q'\sim P''$ for all $w_2(Q',P'')>0$,
	\item[b)] $\Delta_2(Q')=\Sigma_{P''\in\mathcal{P}}w_2(Q',P'')$ for all $Q'\in \mathcal{P}$, and
	\item[c)] $\Delta_3(P'')=\Sigma_{Q'\in\mathcal{P}}w_2(Q',P'')$ for all $P''\in \mathcal{P}$.
\end{enumerate}
Then we have the following calculations:
$$\begin{array}{lclr}
	\Theta&=&\Sigma_{Q'\in\lceil\Delta_2\rceil}\Delta_2(Q')\delta(Q'\backslash L)&  \\
	&=&\Sigma_{Q'\in\mathcal{P}}\Delta_2(Q')\delta({Q'\backslash L})& \mbox{$\Delta_2(Q')=0$
		for $Q'\notin\lceil\Delta_2\rceil$}\\
	&=&
	\Sigma_{Q'\in\mathcal{P}}(\Sigma_{P''\in\mathcal{P}}w_2(Q',P''))\delta({Q'\backslash L})&\mbox{above b)}\\
	&=&
	\Sigma_{Q'\in\mathcal{P},P''\in\mathcal{P}}w_2(Q',P'')\delta({Q'\backslash L})\\
	&=&
	\Sigma_{Q' \sim P''}w_2(Q',P'')\delta({Q'\backslash L})&\mbox{$w_2(Q',P'')=0$ for $(Q',P'')\not\sim S $}\\
\end{array}
$$
Similarly, we can obtain $\Theta'=\Sigma_{Q'\sim P''}w_2(Q',P'')\delta({P''\backslash L})$, thus $\Theta\sim^\dagger\Theta'$.
Hence $\Delta S^\dagger \Theta' (\sim)^\dagger \Theta$ by Proposition~\ref{Prolift}, that is $\Delta\, ( S\,\cdot\sim)^\dagger\Theta$, as required.\\

\textbf{6) $G\equiv G_1[f]$.} The proof of this case follows the same lines as that of case 5) above, and thus we omit the details.
\end{proof}


==> Secs/6-Thealternating-bitprotocol.tex <==
\section{Verification of Alternating-Bit Protocol} \label{sec7}
The Alternating-Bit Protocol is one of the most studied verification examples
in process algebra. The protocol is used to send and receive information over unreliable channels via an acknowledgment-based mechanism. Its name reflects the method it employs, where bits 0 and 1 are alternately appended to both the transmitted data and the acknowledgment messages. Both the transmitted data and the acknowledgment messages can be lost, or duplicated,
but not altered
in the channel during transmission. In this version of the Alternating-Bit Protocol, we introduce probabilistic information to the transmission channels, thus endowing the protocol with both nondeterministic and probabilistic characteristics. This version of the protocol consists of four separate processes that communicate with each other. Here for a bit $b$ we write $\hat b$
for its opposite, i.e. $\hat 1=0$ and $\hat 0=1$. In the formula below, $a,b\in\{0,1\}$, and $s,t\in\{0,1\}^*$.

Sender:
$$\begin{array}{rcl}
Send(b)&\mathop{=}\limits^{\rm def}&\overline{send_b}. \langle1\rangle{Sending(b)}\\
Sending(b)&\stackrel{\rm def}{=}&\tau.\langle1\rangle Send(b)+ack_b.\langle1\rangle Accept(\hat{b})
+ack_{\hat{b}}.\langle1\rangle Sending(b)\\
Accept(b)&\mathop{=}\limits^{\rm def}&accept.\langle1\rangle Send(b).
\end{array}
$$
The Sender process has three states.
\begin{enumerate}
\item
In the state $Send(b)$ it sends a message
through port ${send_b}$ (for simplicity here we omit the message itself), and afterwards it
goes into state ${Sending(b)}$ with probability $1$.
\item In the state ${Sending(b)}$ it can non-deterministically
go back to ${Send(b)}$ state, which means it will resend the message that is presently being sent;
or if it receives acknowledgement from port $ack_b$ (which means that the message which is being sent has been received
by the Replier), then it goes into state $Accept(\hat{b})$ with probability $1$; or if it
receives acknowledgement from port $ack_{\hat b}$ (which means that it is the acknowledgement of the last
sent message), then in this case it ignores the acknowledgement and
remains in the present state with probability $1$ to continue sending the
present message.
\item In the state $Accept(b)$ it is ready to accept a new message through port $accept$, and afterwards
goes into state $send(b)$ with probability $1$ to send the message.
\end{enumerate}

Replier:
$$\begin{array}{rcl}
Reply(b)&\mathop{=}\limits^{\rm def}&\overline{reply_b}.\langle1\rangle Replying(b)\\
Replying(b)&\mathop{=}\limits^{\rm def}&\tau.\langle1\rangle Reply(b)+trans_{\hat{b}}.\langle1\rangle Deliver(\hat{b})+
trans_b.\langle1\rangle Replying(b)\\
Deliver(b)&\mathop{=}\limits^{\rm def}&\overline{deliver}.\langle1\rangle Reply(b).
\end{array}$$

The Replier process also has three states.
\begin{enumerate}
\item
In the state $Reply(b)$ it sends $b$
through the port ${reply_b}$ signalling that the message with bit $b$ has been received, and afterwards it
goes into state ${Replying(b)}$ with probability $1$.
\item In the state ${Replying(b)}$ it can non-deterministically
go back to ${Reply(b)}$ state, which means it will resend the bit $b$ that is presently being sent;
or if it receives a message from port $trans_{\hat b}$ (which means that it is a new message),
then it goes into state $Deliver(\hat{b})$ with probability $1$; or if it
receives a message from port $trans_{b}$ (which means that it is the message that has just been received
and is acknowledging at present),
then in this case it ignores the message and
remains in the present state with probability $1$ to continue acknowledging the
message that has been received.
\item In the state $Deliver(b)$ it will deliver the received message at port $deliver$
and then go into state $Reply(b)$  to acknowledge receiving the message with probability $1$.
\end{enumerate}

Transmission:
$$\begin{array}{rcl}
Trans(\epsilon)&\mathop{=}\limits^{\rm def}&send_b.\langle1\rangle Trans(b)+send_{\hat{b}}.\langle1\rangle Trans(\hat{b})\\
Trans(sa)&\mathop{=}\limits^{\rm def}&send_b.\langle1\rangle Trans(bsa)+send_{\hat{b}}.\langle1\rangle Trans(\hat{b}sa)+
\overline{trans_a}.\langle1\rangle Trans(s)\\
&&+\tau.\biguplus_{i=1}^{|sa|}(\langle \frac{1}{2|sa|}\rangle Trans(i^+(sa))\uplus
\langle \frac{1}{2|sa|}\rangle Trans(i^-(sa)))
\end{array}$$
where $i^+(t)$ is the string which is the result of duplicating the $i$-th bit of $t$ (for example
$2^+(010)=0110$), and $i^-(t)$ is the string which is the result of deleting the $i$-th bit of $t$,
and $|t|$ is the length of $t$.


The states of the transmission line Transmission is parameterized by the content that is currently in the line.
\begin{enumerate}
\item
When the line is empty (i.e. it contains empty string) it is in the state $Trans(\epsilon)$, and in this
state it can only accept a message to transmit at port $send_b$ or $send_{\hat b}$, and afterwards the state of the line
becomes $Trans(b)$ or $Trans(\hat b)$ accordingly with probability $1$.
\item
When the line is not empty, then it is in a state $Trans(sa)$ where $a\in\{0,1\}$ and $s\in\{0,1\}^*$, that
is $sa$ are the messages in the line being transmitted. In this state
it can either add a new message to transmit at port $send_b$ or $send_{\hat b}$, and afterwards the state of the line
becomes $Trans(bsa)$ or $Trans(\hat bsa)$ accordingly with probability $1$, or it can transmit the first message in
line, i.e. $a$ and change the state to $Trans(s)$ afterwards with probability $1$, or it can silently duplicate
or lose some message in the line, and afterwards change to the corresponding state with probability $\frac{1}{2|sa|}$.
The particular probability $\frac{1}{2|sa|}$ is based on the fact that there are total $|sa|$ positions that error
can occur, with each position two different possible errors (duplicating or losing), and assuming equal chance for
all errors.
\end{enumerate}

Acknowledgment:
$$\begin{array}{rcl}
Ack(\epsilon)&\mathop{=}\limits^{\rm def}&reply_b.\langle1\rangle Ack(b)+reply_{\hat{b}}.\langle1\rangle Ack(\hat{b})\\
Ack(as)&\mathop{=}\limits^{\rm def}&reply_b.\langle1\rangle Ack(asb)+
reply_{\hat b}.\langle1\rangle Ack(as\hat b)+\overline{ack_a}.\langle1\rangle Ack(s)\\
&&+\tau.\biguplus_{i=1}^{|as|}(\langle \frac{1}{2|as|}\rangle Ack(i^+(as))\uplus\langle \frac{1}{2|as|}\rangle Ack(i^-(as))).
\end{array}$$
The states of Acknowledgement is the dual of that of Transmission.


The complete system is built by the above four parts as follows:
$$\begin{array}{rcl}AB\mathop{=}\limits^{\rm def}Accept(\hat{b})||Trans(\epsilon)||Ack(\epsilon)||Reply(b).
\end{array}$$
where $||$ denotes restricted Composition where the ports
$$ack_1,ack_0,reply_1,reply_0,send_1,send_0,trans_1,trans_0$$
are restricted from outside. The initial state of $AB$ is that
a message has just been delivered, a new message is just about to be accepted, and the Transmission and  Acknowledgment are empty.

And, we define the protocol specification to be a buffer as follows:
$$\begin{array}{rcl}
\mbox{\em Buff}&\mathop{=}\limits^{\rm def}&accept.\langle1\rangle\mbox{\em Buff\,}'\\
\mbox{\em Buff\,}'&\mathop{=}\limits^{\rm def}&\overline{deliver}.\langle1\rangle\mbox{\em Buff}.
\end{array}$$
To prove that $AB$ meets its specification, we will show that
$$AB\approx_{b}\mbox{\em Buff}.$$
For that we will apply the bisimulation verification technique by constructing a branching bisimulation which
contains $(AB,\mbox{\em Buff})$.

Figure \ref{fig1} shows a binary relation $\mathcal{S}_{b}$ which contains $(AB,\mbox{\em Buff})$, and which is
 partitioned into twelve groups indexed by $m,n,p,q\geq 0$ and by $b\in\{0,1\}$.
\begin{figure*}[h]
	\centering
	\begin{equation}
		\begin{aligned}
        &AB\text{ states}&\mbox{\em Buff}&\text{ states}\\
        &Accept(\hat{b})||Trans(b^n)||Ack(b^p)||\left\{\begin{array}{rcl}&Reply(b)\\&Replying(b)\end{array}\right. &\mbox{\em Buff}\\
        &\left.\begin{array}{rcl}Send(\hat{b})\\Sending(\hat{b})\end{array}\right\}  ||Trans(\hat{b}^mb^n)||Ack(b^p)||\left\{\begin{array}{rcl}&Reply(b)\\&Replying(b)\end{array}\right. &\mbox{\em Buff\,}'\\
        &\left.\begin{array}{rcl}Send(\hat{b})\\Sending(\hat{b})\end{array}\right\}  ||Trans(\hat{b}^m)||Ack(b^p)||Deliver(\hat{b}) &\mbox{\em Buff\,}'\\
        &\left.\begin{array}{rcl}Send(\hat{b})\\Sending(\hat{b})\end{array}\right\}  ||Trans(\hat{b}^m)||Ack(b^p\hat{b}^q)||\left\{\begin{array}{rcl}&Reply(\hat{b})\\&Replying(\hat{b})\end{array}\right. &\mbox{\em Buff}
		\end{aligned}\nonumber
	\end{equation}
  \caption{The binary relation $\mathcal{S}_{b}$}\label{fig1}
 \end{figure*}

The twelve groups arise by choosing either of each pair of bracketed alternatives. We can check that
$\mathcal{S}_{b}\cup\mathcal{S}_{b}^-$ is a branching bisimulation.
To this end, let us start by considering one group of pairs, say the pairs
$$(Sending(\hat{b}) ||Trans(\hat{b}^mb^n)||Ack(b^p)||Reply(b), \mbox{\em Buff\,}')\in\mathcal{S}_{b}$$
for all values of the bit $b$ and the integers $m,n$ and $p$.
Consider the actions of the left member.
\begin{itemize}
\item[(1)] There are $\tau$ actions corresponding to loss or duplication by $Trans$ or $Ack$:
    $$\begin{array}{rcl}
    Trans(\hat{b}^mb^n)&\arrow{\tau}&
    \Sigma_{i=1}^{m+n}(\frac{1}{2(m+n)}\delta(Trans(i^+(\hat{b}^mb^n)))+
    \frac{1}{2(m+n)}\delta(Trans(i^-(\hat{b}^mb^n))))\\
    Ack(b^p)&\arrow{\tau}&\Sigma_{i=1}^{p}(\frac{1}{2p} \delta(Ack(i^+(b^p)))+\frac{1}{2p}\delta (Ack(i^-(b^p))))
    \end{array}$$
    After calculation according to the definition of $i^+$ and $i^-$, we have that
    $$\begin{array}{rcl}
    Trans(\hat{b}^mb^n)&\arrow{\tau}&
    \left.\begin{array}{rcl}\frac{m}{2(m+n)}\delta( Trans(\hat{b}^{m-1}b^n)) +\frac{m}{2(m+n)}\delta( Trans(\hat{b}^{m+1}b^n))+\\ \frac{n}{2(m+n)} \delta (Trans(\hat{b}^{m}b^{n-1})) +\frac{n}{2(m+n)}\delta( Trans(\hat{b}^{m}b^{n+1})) \end{array}\right.\\
    Ack(b^p)&\arrow{\tau}&\frac{1}{2}\delta( Ack(b^{p+1}))+ \frac{1}{2}\delta( Ack(b^{p-1}))
    \end{array}$$
    The derivatives of those actions belong to the same group, and we have
    $\mbox{\em Buff\,}'\dobarrow{}_c\delta(\mbox{\em Buff\,}')$ and
    $\mbox{\em Buff\,}'\arrow{(\tau)}_c\delta(\mbox{\em Buff\,}')$ to match these transitions, since
    %$$\delta(Trans(\hat{b}^kb^l))(\mathcal{S}_{b})^\dagger\delta(\mbox{\em Buff\,}')$$
    $$\delta(Sending(\hat{b}) ||Trans(\hat{b}^kb^l)||Ack(b^q)||Reply(b))(\mathcal{S}_{b})^\dagger\delta(\mbox{\em Buff\,}')$$
    for $(k,l)\in\{(m,n),(m-1,n),(m+1,n),(m,n-1),(m,n+1)\}$ and $q\in\{p,p+1,p-1\}$.

    %choose $\mbox{\em Buff\,}'$ again as the corresponding $\tau$-descendant of $\mbox{\em Buff\,}'$.
\item[(2)] The $\tau$ action
    $$\begin{array}{rcl}
    Sending(\hat{b})\arrow{\tau}\delta( Send({\hat{b}}))
    \end{array}$$
    takes us into another group, also paired with $\mbox{\em Buff\,}'$ (its own $\tau$-descendant).
\item[(3)] The $\overline{ack_b}$ action by $Sending(b)$ complements the $ack_b$ action of $Ack(b^p)(p>0)$, yielding a $\tau$-action returning to the same group, and again we choose $\mbox{\em Buff\,}'$ as descendant.
\item[(4)] Finally, the $\overline{reply_b}$ action by $Reply(b)$ complements the $reply_b$ action of $Ack(b^n)$, taking us into another group paired with $\mbox{\em Buff\,}'$(its own $\tau$-descendant).
\end{itemize}
On the other hand, consider
$$(\mbox{\em Buff\,}',Sending(\hat{b}) ||Trans(\hat{b}^mb^n)||Ack(b^p)||Reply(b))\in\mathcal{S}_{b}^-$$
and the only action of $\mbox{\em Buff\,}'$ is
$$\begin{array}{rcl}
\mbox{\em Buff\,}'\arrow{\overline{deliver}}\delta(\mbox{\em Buff}),
\end{array}$$
 which can be matched as follows:
 by allowing $Reply(b)$ to do $\overline{reply_b}$, then do $trans_b$ $n$ times, then $trans_{\hat{b}}$
  - all these yielding $\tau$-actions of the right member to arrive at state
  $$Sending(\hat{b}) ||Trans(\hat{b}^{m-1})||Ack(b^{p+1})||Deliever(\hat{b}),$$
  which finally perform $\overline{deliver}$, yielding the $\overline{deliver}$-descendant
$$\begin{array}{rcl}
Sending(\hat{b}) ||Trans(\hat{b}^{m-1})||Ack(b^{p+1})||Reply(\hat{b}).
\end{array}$$
  That is
  $$\begin{array}{l}
  Sending(\hat{b}) ||Trans(\hat{b}^mb^n)||Ack(b^p)||Reply(b))\dobarrow{}_c\\
  \delta(Sending(\hat{b}) ||Trans(\hat{b}^{m-1})||Ack(b^{p+1})||Deliever(\hat{b}))
  \end{array}
  $$
  and
$$\begin{array}{l}
Sending(\hat{b}) ||Trans(\hat{b}^{m-1})||Ack(b^{p+1})||Deliever(\hat{b})\arrow{\overline{deliver}}\\
\delta(Sending(\hat{b}) ||Trans(\hat{b}^{m-1})||Ack(b^{p+1})||Reply(\hat{b})),
\end{array}$$
and the transitions match
$$\begin{array}{rcl}
\mbox{\em Buff\,}'\arrow{\overline{deliver}}\delta(\mbox{\em Buff})
\end{array}$$
because
$$\delta(\mbox{\em Buff\,}')(\mathcal{S}_{b}\cup\mathcal{S}_{b}^-)^\dagger\delta(Sending(\hat{b}) ||Trans(\hat{b}^{m-1})||Ack(b^{p+1})||Deliever(\hat{b}))
$$
and
$$\delta(\mbox{\em Buff})(\mathcal{S}_{b}\cup\mathcal{S}_{b}^-)^\dagger
\delta(Sending(\hat{b}) ||Trans(\hat{b}^{m-1})||Ack(b^{p+1})||Reply(\hat{b})).
$$

By similar exhaustive case analysis, it can indeed be verified that $\mathcal{S}_{b}\cup\mathcal{S}_{b}^-$ is a branching bisimulation.


==> Secs/6ConsistentExtensionOfCCS.tex <==

\section{A Consistent Extension of CCS} \label{sec6}

In this section we will show that the strong and branching bisimilarities that we have defined for
probabilistic processes extends the corresponding notions of equivalence for non-probabilistic processes of CCS.
First we recall the syntax and semantics of CCS.

The set of CCS processes, denoted $\mathcal{P}_{\sf ccs}$, is given by the following BNF rules
$$
\begin{array}{ccc|c|c|c|c|c}
	P&::=&\alpha.P&\sum_{i\in I}P_{i}&P\mathbin{|}P&P[f]& P\backslash L &A
\end{array}
$$
where we use the same conventions as in Section \ref{sec2}.

The operational semantics of the CCS processes is given by a transition relation
$$\arrow{}_{\sf ccs}\subseteq\mathcal{P}_{\sf ccs}\times{Act}\times\mathcal{P}_{\sf ccs}$$
by the usual rules, such as:
\begin{equation*}
	\nonumber
	\begin{aligned}
		& \alpha.P \arrow{\alpha}_{\sf ccs} P \quad \frac{\displaystyle P_j \arrow{\alpha}_{\sf ccs} P_j'}{\displaystyle \Sigma_{i\in I} P_i \arrow{\alpha}_{\sf ccs} P_j'} \quad (j \in I) \\
		& \frac{\displaystyle P \arrow{\alpha}_{\sf ccs} P'}{\displaystyle P | Q \arrow{\alpha}_{\sf ccs} P' | Q} \quad \ldots
	\end{aligned}
\end{equation*}
%\begin{array}{rlrl}
%\mbox{}\ \ \ \ \ \ &\frac{\displaystyle P\arrow{\alpha}_{\sf ccs}P'}{\displaystyle P|Q\arrow{\alpha}_{\sf ccs}
%P'|Q}{}\ \ \ \ \ \ \
%&\mbox{}\ \
%&\frac{\displaystyle Q\arrow{\alpha}\Delta}{\displaystyle P|Q\arrow{\alpha}
%\Sigma_{O\in\lceil\Delta\rceil}\Delta(O)\delta({P|O})}{}
%\end{array}\\
%\begin{array}{rl}&\frac{\displaystyle P\arrow{l}\Delta\ \
%Q\arrow{\bar l}\Theta}{\displaystyle P|Q\arrow{\tau}
%\Sigma_{(U,V)\in\lceil\Delta\rceil\times\lceil\Theta\rceil}(\Delta(U)\cdot\Delta(V))\delta({U|V})}{}
%\end{array}\\
%\begin{array}{rlrl}& \frac{\displaystyle P\arrow{\alpha}\Delta}{\displaystyle P[f]\arrow{f(\alpha)}
%\Sigma_{O\in\lceil\Delta\rceil}\Delta(O)\delta({O[f]})}{}\ \ \ \ \ \ %\ \ \
%&
%& \frac{\displaystyle P\arrow{\alpha}\Delta}{\displaystyle A\arrow{\alpha}\Delta}
%{\ \ (A\stackrel{{\rm def}}{=}P)}
%\end{array}\\
%\begin{array}{rl}
%& \frac{\displaystyle P\arrow{\alpha}\Delta}{\displaystyle P\backslash L\arrow{\alpha}
%\Sigma_{O\in\lceil\Delta\rceil}\Delta(O)\delta({O\backslash L})}
%{\ \ (\alpha,\overline\alpha\notin L)}\end{array}
In keeping with tradition, we also define the relation $\dobarrow{}_{\sf ccs}$. Specifically, $P\dobarrow{}_{\sf ccs}Q$ denotes that process P can evolve into process Q through a sequence of zero or more internal actions.

Strong and branching bisimilarities are defined as follows.

\begin{definition} A symmetric  binary relation $R\subseteq\mathcal{P}\times\mathcal{P}$ is a
{\em strong bisimulation} if $PR\,Q$ implies the following:
whenever $P\arrow{\alpha}_{\sf ccs}P'$ for some $\alpha\in{Act}$ and $P'\in{\mathcal P}_{\sf ccs}$,
then $Q\arrow{\alpha}_{\sf ccs}Q'$ for some $Q'$ such that
$P'R\,Q'$.

We say that two processes $P,Q\in\mathcal{P}_{\sf ccs}$ are strong bisimilar, written $P\sim_{\sf ccs}Q$,
if there is a strong bisimulation $R$ such that $PR\,Q$.

A symmetric  binary relation $R\subseteq\mathcal{P}_{\sf ccs}\times\mathcal{P}_{\sf ccs}$ is a
{\em branching bisimulation} if $PR\,Q$ implies the following:
whenever
$P\arrow{\alpha}_{\sf ccs}P'$ for some $\alpha\in{Act}$ and $P'\in{\mathcal P}_{\sf ccs}$,
then $Q\dobarrow{}_{\sf ccs}Q'$ for some $Q'$ such that $Q'\arrow{(\alpha)}_{\sf ccs}Q''$ for some
$Q''\in{\mathcal P}_{\sf ccs}$ such that $PR\,Q'$ and $P'R\,Q''$.

We say that two processes $P,Q\in\mathcal{P}_{\sf ccs}$ are branching bisimilar, written
$P\approx_{b{\sf ccs}}Q$,
if there is a branching bisimulation $R$ such that $PR\,Q$.
\end{definition}

Now we can define a map $\lbrack\underline{\ }\rbrack$ which
takes a CCS process $P\in\mathcal{P}_{\sf ccs}$ to a process
$[P]\in\mathcal{P}$. $\lbrack\underline{\ }\rbrack$ is defined  by induction on the structure of $P$
as follows:
$$\begin{array}{ccc}
[\alpha.P]\equiv\alpha.\langle 1\rangle[P],&[\Sigma_{i\in I}P_i]\equiv \Sigma_{i\in I}[P_i],&[P|Q]\equiv[P]|[Q],\\

[P{[f]}]\equiv[P][f],&[P\backslash L]\equiv[P]\backslash L,& [A]\equiv A
\end{array}
$$

The main objective of this section is to demonstrate that probabilistic bisimilarity constitutes a conservative extension of the corresponding equivalence in classical CCS. We begin with Lemma~\ref{Lemma-embedding}, which establishes a correspondence between the transitions of classical CCS processes and those of probabilistic processes; this result is straightforward and its proof is therefore omitted. Building on Lemma~\ref{Lemma-embedding}, we establish Theorem~\ref{Th-correspondance1}, showing that probabilistic bisimilarity is indeed a conservative extension of classical bisimilarity.

\begin{lemma}\label{Lemma-embedding}
	Let $P$ be a CCS process, then $[P]\arrow{\alpha}\Delta$ if and only if there exists a CCS process $Q$ such that
	$P\arrow{\alpha}_{\sf ccs}Q$ and $\Delta=\delta([Q])$.
\end{lemma}
\begin{proof} Routine.
\end{proof}

%Now we can prove some interesting properties about the
%map $[\underline{\ }]$.
\begin{theorem}\label{Th-correspondance1} Let $P,Q\in\mathcal{P}_{\sf ccs}$, then
	$P\sim_{{\sf ccs}} Q$ if and only if $[P]\sim[Q]$.
\end{theorem}
\begin{proof}
	For the "if" direction it is sufficient to show that
	$$R=\setof{(P,Q)}{[P]\sim[Q]}
	$$
	is a strong bisimulation for non-probabilistic processes. Suppose $PR\,Q$ and $P\arrow{\alpha}_{\sf ccs}P'$.
	According to
	Lemma \ref{Lemma-embedding} $[P]\arrow{\alpha}\delta([P'])$. Since $[P]\sim[Q]$, there is $\Theta$ such that
	$[Q]\arrow{\alpha}\Theta$ and $\delta([P'])\sim^\dagger\Theta$. Now according to Lemma \ref{Lemma-embedding}
	there is $Q'$ such that $Q\arrow{\alpha}_{\sf ccs}Q'$ and $\Theta=\delta([Q'])$, thus
	$\delta([P'])\sim^\dagger\delta([Q'])$, so $[P']\sim[Q']$ hence $P'R\,Q'$. This shows that $R$ is a strong bisimulation
	for non-probabilistic processes.
	
	For the "only if" direction it is sufficient to show that
	$$R=\setof{([P],[Q])}{P\sim_{\sf ccs}Q}
	$$
	is a strong bisimulation. 
	\\Suppose $[P]R[Q]$ and $[P]\arrow{\alpha}\Delta$.
	According to
	Lemma \ref{Lemma-embedding} there is $P'$ such that $P\arrow{\alpha}_{\sf ccs}P'$ and $\Delta=\delta([P'])$.
	Since $P\sim_{\sf ccs}Q$, there is $Q'$ such that $Q\arrow{\alpha}_{\sf ccs}Q'$ and $P'\sim_{\sf ccs}Q'$,
	then by Lemma \ref{Lemma-embedding} $[Q]\arrow{\alpha}\delta([Q'])$, moreover since $P'\sim_{\sf ccs}Q'$
	thus $[P']R[Q']$ and $\delta([P'])R^\dagger\delta([Q'])$. This shows that $R$ is a strong bisimulation.
\end{proof}

Next we will prove the branching bisimilarity version of Theorem \ref{Th-correspondance1}, which is less trivial
because of the combined weak transition $\dobarrow{}_c$. The following lemma
makes necessary preparation. 
\begin{lemma}\label{Lemma-ctrans}
	Let $P$ be a CCS process.
	\begin{enumerate}
		\item If $P\dobarrow{}_{\sf ccs}Q$ then $[P]\dobarrow{}_c\delta([Q])$;
		\item If $[P]\dobarrow{}_c\Delta$ then there exists a CCS processes $Q$ such that $[Q]\in\lceil\Delta\rceil$,
		and $P\dobarrow{}_{\sf ccs}Q$.
	\end{enumerate}
\end{lemma}
\begin{proof} The proof of 1. is simple.
	
	The proof of 2. is carried out by induction on the transition $[P]\dobarrow{}_c\Delta$.
	If $\Delta=\delta([P])$, then $P\dobarrow{}_{\sf ccs}P$. If $[P]\dobarrow{}_c\Delta$ is because
	$[P]\arrow{\tau}\Delta$, then by Lemma \ref{Lemma-embedding} there is a CCS process $Q$ such that
	$P\arrow{\tau}_{\sf ccs}Q$ and $\Delta=\delta([Q])$, thus $P\dobarrow{}_{\sf ccs}Q$. If
	$[P]\dobarrow{}_c\Delta$ is because $\Delta=p\Delta'+(1-p)\Delta''$, where
	$[P]\dobarrow{}_cp\delta(P')+(1-p)\Delta''$ and $P'\dobarrow{}_c\Delta'$, then
	by the induction hypothesis there exists a CCS process $Q'$ such that
	$P\dobarrow{}_{\sf ccs}Q'$ and $[Q']\in\lceil p\delta(P')+(1-p)\Delta''\rceil$.
	Then either $[Q']\in\lceil\Delta''\rceil$, in this case $[Q']\in\lceil\Delta\rceil$ and
	we are done, or $[Q']\in\lceil\delta(P')\rceil$, in this case $P'$ is $[Q']$, thus
	$[Q']\dobarrow{}_c\Delta'$,
	again by the induction hypothesis there exists a CCS process
	$Q$ such that $Q'\dobarrow{}_{\sf ccs}Q$ and $[Q]\in\lceil\Delta'\rceil$, now
	$P\dobarrow{}_{\sf ccs}Q$ and $[Q]\in\lceil\Delta\rceil$
	we are done.
\end{proof}

\begin{theorem} \label{Th-correspondance2} Let $P,Q\in\mathcal{P}_{\sf ccs}$, then
	$P\approx_{b{\sf ccs}} Q$ if and only if $[P]\approx_b[Q]$.
\end{theorem}
\begin{proof}
	For the "if" direction it is sufficient to show that
	$$R=\setof{(P,Q)}{[P]\approx_b[Q]}
	$$
	is a branching bisimulation for non-probabilistic processes. Suppose $PR\,Q$ and $P\arrow{\alpha}_{\sf ccs}P'$.
	According to
	Lemma \ref{Lemma-embedding} $[P]\arrow{\alpha}\delta([P'])$. Since $[P]\approx_b[Q]$, there is $\Theta$ such that
	$[Q]\dobarrow{}_c\Theta$ and $\delta([P])(\approx_b)^\dagger\Theta$, and moreover
	for every $O\in\lceil\Theta\rceil$ it holds that $O\arrow{(\alpha)}\Theta'$ for some $\Theta'$
	with $\delta([P'])(\approx_b)^\dagger\Theta'$. Now according to 2. of Lemma \ref{Lemma-ctrans}
	there is $Q'$ such that $Q\dobarrow{}_{\sf ccs}Q'$ and $[Q']\in\lceil\Theta\rceil$, thus $[Q']\arrow{(\alpha)}\Theta'$
	for some $\Theta'$ with $\delta([P'])(\approx_b)^\dagger\Theta'$,
	from $\delta([P])(\approx_b)^\dagger\Theta$ it follows that $[P]\approx_b[Q']$, so $P R\,Q'$,
	and from $[Q']\arrow{(\alpha)}\Theta'$ by Lemma \ref{Lemma-embedding} there is a CCS process $Q''$
	such that $Q'\arrow{(\alpha)}Q''$ and $\Theta'=\delta([Q''])$, thus $\delta([P'])(\approx_b)^\dagger\delta([Q''])$
	and so $[P']\approx_b[Q'']$ which implies $P'R\,Q''$.
	This shows that $R$ is a branching bisimulation
	for non-probabilistic processes.
	
	For the "only if" direction it is sufficient to show that
	$$R=\setof{([P],[Q])}{P\approx_{b{\sf ccs}}Q}
	$$
	is a branching bisimulation. Suppose $[P]R[Q]$ and $[P]\arrow{\alpha}\Delta$.
	According to
	Lemma \ref{Lemma-embedding} there is $P'$ such that $P\arrow{\alpha}_{\sf ccs}P'$ and $\Delta=\delta([P'])$.
	Since $P\approx_{b{\sf ccs}}Q$, there exist $Q',Q''$ such that $Q\dobarrow{}_{\sf ccs}Q',
	Q'\arrow{(\alpha)}_{\sf ccs}Q''$ and $P\approx_{b{\sf ccs}}Q', P'\approx_{b{\sf ccs}}Q''$,
	then by 1. of Lemma \ref{Lemma-ctrans} $[Q]\dobarrow{}_c\delta([Q'])$ and $\delta([P])R^\dagger\delta([Q'])$
	(since $P\approx_{b{\sf ccs}}Q'$ thus $[P]R[Q']$), moreover $[Q']$ is the only element in $\lceil\delta([Q'])\rceil$,
	and $[Q']\arrow{(\alpha)}\delta([Q''])$, $\delta([P'])R^\dagger\delta([Q''])$ (since $P'\approx_{b{\sf ccs}}Q''$
	thus $[P']R[Q'']$), this shows that $R$ is a branching bisimulation.
\end{proof}

Then in a very precise sense the map $[\underline{\ }]$ is an embedding of the branching bisimulation theory
about CCS processes into the branching bisimulation theory about probabilistic processes studied in this paper. Or
in other words, the work presented in this paper is a consistent extension of the related work about branching bisimulation
of non-probabilistic processes.




